Improving Cross-Lingual Token Representations by Adding a Pinch of SALT

Cross-lingual sentence encoders enable scalable transfer across hundreds of languages, powering applications such as translation mining and zero-shot learning in low-resource settings. Although trained for sentence-level alignment, they are increasingly also applied to token-level tasks such as hallucination detection and sequence tagging, exposing a mismatch between training and usage. We propose SALT, a lightweight post-training method that improves token representations by injecting span-level supervision into existing sentence encoders. Across five multilingual token-level benchmarks, SALT achieves the best overall results on four of them, outperforming alternative fine-tuning strategies and competitive encoders. It also improves sentence-level performance on cross-lingual retrieval and classification tasks. These results demonstrate that span-level supervision is an effective signal for improving both token and sentence representations.

==> SALT/latex/1_intro.tex <==
\begin{figure*}[t]
  \centering
  \resizebox{0.9\textwidth}{!}{%
    \begin{tikzpicture}[
      >=Stealth, font=\small,
      encoder/.style={draw,rounded corners=4pt,fill=encodergreen!70,minimum width=1.8cm,minimum height=1.0cm,align=center,font=\small\bfseries},
      decoder/.style={draw,rounded corners=4pt,fill=decoderpink,minimum width=1.8cm,minimum height=1.0cm,align=center,font=\small\bfseries},
      loss/.style={draw,rounded corners=2pt,fill=white,minimum width=2.0cm,minimum height=0.7cm,align=center,font=\small},
      emb/.style={draw=gray!60,rounded corners=1pt,fill=#1,minimum width=0.26cm,minimum height=1.4cm},
      embsm/.style={draw=gray!60,rounded corners=1pt,fill=#1,minimum width=0.26cm,minimum height=1.0cm},
      sent/.style={draw=gray!50,rounded corners=3pt,fill=#1,minimum height=0.6cm,inner xsep=5pt,font=\small,align=center}
    ]

    %% Section headers
    \node[font=\large\bfseries, anchor=west] at (-9.5, -0.3) {Pre-processing};
    \node[font=\small, anchor=center] at (0.5, -0.7) {Span alignment extraction};

    %% Full sentences
    \node[sent=myyellow!50, minimum width=8.5cm] (en-full) at (-4.0, -1.4)
      {with your age, all chest pain should be treated this way};
    \node[sent=mypurple!35, minimum width=8.5cm] (es-full) at (-4.0, -2.3)
      {a su edad el dolor de pecho debe tratarse de esta manera};

    \draw[->, thick] (0.30, -1.85) -- (1.05, -1.85);

    %% English spans
    \node[sent=myblue, text=white, anchor=west, minimum width=2.2cm] at (1.15,-1.4) {with your age};
    \node[sent=mylightblue, anchor=west, minimum width=0.9cm] at (3.53,-1.4) {, all};
    \node[sent=mygreen!60, anchor=west, minimum width=1.9cm] at (4.51,-1.4) {chest pain};
    \node[sent=myyellow!80, anchor=west, minimum width=2.9cm] at (6.49,-1.4) {should be treated};
    \node[sent=myorange!70, anchor=west, minimum width=1.4cm] at (9.47,-1.4) {this way};

    %% Spanish spans
    \node[sent=myblue, text=white, anchor=west, minimum width=1.8cm] at (1.15,-2.3) {a su edad};
    \node[sent=mygreen!60, anchor=west, minimum width=2.8cm] at (3.03,-2.3) {el dolor de pecho};
    \node[sent=myyellow!80, anchor=west, minimum width=2.3cm] at (5.91,-2.3) {debe tratarse};
    \node[sent=myorange!70, anchor=west, minimum width=2.3cm] at (8.29,-2.3) {de esta manera};

    %% Single frozen encoder
    \node[encoder] (enc-top) at (-2.5,-4.0) {Encoder};
    \snowflake{-2.5+0.6}{-3.57-0.15}{0.03}
\draw[->] (es-full.south) -- ++(0,-1.35) |- (enc-top.west);
   % \draw[->] (en-full.south) -- ++(0,-0.25) -| (enc-top.north);

   
    \draw[->] (enc-top.east) -- node[above,font=\small,align=center]{Sentence-level\\representation} (1.5,-4.0);

    %% Teacher embedding: yellow + purple = blue
    \foreach \i in {1}{ \node[emb=myyellow!70] at (2.0+\i*0.30-0.30,-4.0) {}; }
    \node[font=\normalsize] at (2.32,-4.0) {$+$};
    \foreach \i in {1}{ \node[emb=mypurple!50] at (2.65+\i*0.30-0.30,-4.0) {}; }
    \node[font=\normalsize] at (2.97,-4.0) {$=$};
    \foreach \i in {1}{ \node[emb=myblue!60] at (3.3+\i*0.30-0.30,-4.0) {}; }
    \node[font=\small,align=left] at (4.4,-4.0) {Teacher\\embedding};






    %% Divider + Training header
    \draw[gray,line width=0.6pt] (-9.5,-5.1) -- (11.5,-5.1);
    \node[font=\large\bfseries,anchor=west] at (-9.5,-5.6) {Training};
     \salttikz{-7.3}{-5.6}{0.05}
    


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%
%%%%%%%  BOTTOM PART

    %% Bottom sentences
    \node[sent=mypurple!35,minimum width=8.5cm] (es-bot) at (-4.5,-6.5)
      {a su edad el dolor de pecho debe tratarse de esta manera};
    \node[sent=myyellow!50,minimum width=8.5cm] (en-bot) at (6.5,-6.5)
      {with your age, all chest pain should be treated this way};

    %% Trainable encoders
    \node[encoder] (enc-bot-L) at (-4.5,-7.7) {Encoder};
    \flame{-4.82+0.9}{-7.33}{0.03}
    \node[encoder] (enc-bot-R) at (6.5,-7.7) {Encoder};
    \flame{6.18+0.9}{-7.33}{0.03}
    \draw[->] (es-bot.south) -- (enc-bot-L.north);
    \draw[->] (en-bot.south) -- (enc-bot-R.north);

    %% Token embeddings (Spanish)
    \foreach \i in {1,...,7}{ \node[embsm=mypurple!40] at (-7.2+\i*0.5,-9.1) {}; }

    \node[font=\tiny, scale=0.2] at ({-9.15+9*0.5},-9.5) {$\cdots$};
\foreach \word/\i in {a/1,su/2,edad/3,el/4,dolor/5,de/6,pecho/7}{
  \node[font=\tiny, scale=0.8, anchor=base] 
  at ({-7.2+\i*0.5},-8.45) {\word};}
\node[font=\tiny, scale=0.8, anchor=base] at (-3.0,-8.45) {manera};
    
    \draw[decorate,decoration={brace,amplitude=4pt,mirror}] (-6.80,-9.70) -- (-5.6,-9.70);

    \draw[decorate,decoration={brace,amplitude=4pt,mirror}] (-5.30,-9.70) -- (-3.6,-9.70);

    \foreach \i in {1}{\node[embsm=mypurple!40] at (-3.0,-9.1) {}; }
        
    %\draw[->] (enc-bot-L.south) -- (-4.5,-8.72) -- (-7.85,-8.72) -- (-7.85,-8.74);


%%% RIGHT PART
    %% Token embeddings (English)
    \foreach \i in {1,...,7}{ \node[embsm=myyellow!70] at (3.8+\i*0.5,-9.1) {}; }
      \node[font=\tiny, scale=0.2] at ({-9.15+11+9*0.5},-9.5) {$\cdots$};
      
    \foreach \word/\i in {with/1,your/2,age/3,{,}/4,all/5,chest/6,pain/7}{
  \node[font=\tiny, scale=0.8, anchor=base] 
  at ({-7.2+11+\i*0.5},-8.45) {\word};}
\node[font=\tiny, scale=0.8, anchor=base] at (-3.0+11,-8.45) {way};


    \draw[decorate,decoration={brace,amplitude=4pt,mirror}] (-6.80+11,-9.70) -- (-5.6+11,-9.70);

    \draw[decorate,decoration={brace,amplitude=4pt,mirror}] (5.7,-9.70) -- (6.4,-9.70);

    \draw[decorate,decoration={brace,amplitude=4pt,mirror}] (6.7,-9.70) -- (7.4,-9.70);


    \foreach \i in {1}{\node[embsm=myyellow!70] at (-3.0+11,-9.1) {}; }

    %% Average pool labels + arrows
    \node[font=\small] (avgL) at (-1.3,-8.85) {Average pool};
    %\node[font=\small] (avgR) at (1.8,-8.5) {Average pool};
    \draw[->] (-2.7, -9) -- (0+1, -9) -- (-0+1,-9.45);
    \draw[->] (4.0, -9) -- (0.6+1, -9) -- (0.6+1,-9.45);

    %% L_Teacher = MSE( purple+yellow , blue )
    \node[font=\small] at (-1.30+1.0,-10.1) {$L_{\mathit{INT}}{=}\mathit{MSE}($};
    \foreach \i in {1}{ \node[emb=mypurple!50] at (1+0.02+\i*0.30-0.30,-10.1) {}; }
    \node[font=\normalsize] at (1+0.3,-10.1) {$+$};
    \foreach \i in {1}{ \node[emb=myyellow!70] at (1+0.6+\i*0.30-0.30,-10.1) {}; }
    \node[font=\normalsize] at (1+0.85,-10.1) {$,$};
    \foreach \i in {1}{ \node[emb=myblue!60] at (1+1.1+\i*0.30-0.30,-10.1) {}; }
    \node[font=\normalsize] at (1+1.4,-10.1) {$)$};

    %% Span-aggregated embeddings (Spanish)
    \node[embsm=myblue]     (sp1) at (-6.2,-10.5) {};
    \node[embsm=mygreen!70] (sp2) at (-4.44,-10.5) {};
    \node[font=\small] at (-3.7,-10.8) {$\cdots$};
    \node[embsm=mypink]     (sp3) at (-3.0,-10.5) {};
    \node[align=left,font=\small] at (-7.8,-10.5) {Span-aggregated\\\hspace{10pt}embeddings};
   % \draw[->] (-4.5,-9.55) -- (sp3.east);

    %% Span-aggregated embeddings (English)
    \node[embsm=myblue]     (ep1) at (-6.2+11,-10.5) {};
    \node[embsm=gray!60]    (ep2) at (6.05,-10.5) {};
    \node[font=\small] at (-3.7+11.3,-10.8) {$\cdots$};
    \node[embsm=mygreen!70] (ep3) at (7.05,-10.5) {};
        \node[embsm=mypink]     (sp3) at (-3.0+11,-10.5) {};
   % \draw[->] (6.5,-9.55) -- (6.5,-11.2) -- (ep3.east);

    %% L_CON_SPAN
    \node[font=\small,align=center] at (0.75,-11.65) {Span-based\\contrastive loss};
    \node[loss] (lcspan) at (0.75,-12.5) {$L_{\mathit{CON}_{\mathit{SPAN}}}$};
    \draw[->, dashed, bend right=20] (-4.2, -11.2) to (lcspan.west);
    \draw[->, dashed, bend right=-20] (-4.2+10.5, -11.2) to (lcspan.east);
   % \draw[->,dashed] (ep1.south) -- (4.8,-12.5) -- (lcspan.east);

    %% Decoder + L_MT_SPAN underbrace
    \node[decoder] (decoder) at (-3.5,-13.5) {Decoder};
    %\snowflake{-3.5}{-13.05}{0.22}
    \snowflake{-3.5+0.6}{-13.0-0.2}{0.03}
    \draw[->] (sp1.south) -- (-6.20,-13.5) -- (decoder.west);
    \draw[->] (decoder.east) -- (-2.0,-13.5);
    \node[font=\small] at (-1.0,-13.5) {with your age};
    \draw[decorate,decoration={brace,amplitude=4pt,mirror}]
      (-1.85,-13.7) -- (-0.15,-13.7)
      node[midway,below=5pt,font=\small] {$L_{\mathit{MT}_{\mathit{SPAN}}}$};

    \end{tikzpicture}%
  }
  \caption{\textbf{Pre-processing} (top):
extraction of aligned spans and teacher embeddings from a pre-trained encoder.
           \textbf{Training SALT} (bottom): we train the encoder with span-level contrastive and translation losses to improve token-level representations, besides an interpolation loss that preserves sentence embeddings.}

           \vspace{-5pt}
  \label{diagram}
\end{figure*}



\section{Introduction}

Cross-lingual sentence encoders have become a core building block of multilingual NLP. Models such as SONAR~\citep{sonar} or MEXMA~\citep{mexma} learn a shared embedding space in which semantically equivalent sentences across languages are mapped to nearby representations, leading to strong performance on sentence-level tasks such as cross-lingual retrieval, sentence mining, and zero-shot classification.

Despite being trained for cross-lingual sentence alignment, these models are increasingly used as \emph{token-level representations} in downstream applications, including word alignment~\citep{miao-etal-2024-enhancing}, sequence tagging~\citep{mehta-varma-2023-llm}, hallucination detection~\citep{ottawa}, sentence segmentation~\citep{omnilingualmtteam2026omnilingualmtmachinetranslation} and label projection~\citep{labelproj}. This practice exposes a structural mismatch: sentence encoders are optimised to preserve global semantic similarity, yet are repurposed to support fine-grained token- and phrase-level alignment. As a result, they may yield well-structured sentence embeddings but an inconsistent or noisy token representation.

A promising way to address this mismatch is to introduce training signals at a finer granularity by identifying aligned words across languages and incorporating token-level losses~\citep{alqahtani-etal-2021-using-optimal, miao-etal-2024-enhancing}. However, word-level alignment is often too restrictive, as meaning is frequently distributed across multiple tokens and only fully preserved at the level of phrases rather than individual words.

To this end, we propose using phrases or \emph{spans}—contiguous sequences of tokens that express equivalent meaning across languages. While this alignment signal is implicitly present in parallel data, previous sentence- or token-level objectives do not exploit it. We introduce \salt{0.04} \textbf{SALT} (\textbf{S}pan-\textbf{A}ligned \textbf{L}earning for cross-lingual \textbf{T}okens), a novel lightweight post-training method for multilingual sentence encoders (see Figure~\ref{diagram}). SALT augments standard sentence-level training with span-aligned contrastive and translation objectives that explicitly shape token- and phrase-level representations, while a sentence-level interpolation objective preserves the original embedding space. Importantly, SALT requires no architectural modifications and can be applied directly to existing encoders.
% inductive bias

%OLD We propose that this mismatch can be addressed through additional training signals that operate at a finer granularity. Our key observation is that parallel text contains a rich but underutilised source of supervision beyond sentence-level alignment: translation pairs implicitly define correspondences between \emph{spans}—contiguous sequences of tokens that express equivalent meaning across languages (see Figure~\ref{diagram}). While this signal is implicitly present in the data, it is not explicitly used by standard sentence-level objectives.

%We argue that this missing inductive bias can be exploited to improve token representations without sacrificing sentence-level quality. To this end, we propose \salt{0.04} \textbf{SALT} (\textbf{S}pan-\textbf{A}ligned \textbf{L}earning for cross-lingual \textbf{T}okens), a lightweight post-training method for multilingual sentence encoders. SALT augments standard sentence-level training with span-aligned contrastive and translation objectives that explicitly shape token- and phrase-level representations, while a sentence-level interpolation objective preserves the original embedding space. Importantly, SALT requires no architectural modifications and can be applied directly to existing encoders and decoders.

We evaluate SALT on a suite of multilingual token-level benchmarks, including word alignment, cross-lingual sequence tagging, and word sense disambiguation. Across tasks, SALT consistently improves token-level performance while maintaining or improving sentence-level quality. In particular, it achieves the best overall performance among several fine-tuning strategies on four out of five token-level benchmarks, demonstrating that span-level supervision provides a strong complementary signal rather than a competing objective.

\newpage
Our contributions are as follows:

\begin{itemize}

%\item We identify a structural mismatch between sentence-level training objectives and the token-level usage of multilingual sentence encoders, and show that this leads to suboptimal fine-grained representations.

\item We propose \textbf{SALT}, a lightweight post-training method that injects span-level alignment into sentence encoders, bridging sentence-level training and token-level applications.%\footnote{Model available at [OMIT]. Code available at \href{https://anonymous.4open.science/r/token_local-8E04}{https://anonymous.4open.science/r/token\_local-8E04}.}  

\item We demonstrate that span-aligned supervision consistently improves performance across multiple token-level multilingual tasks, while preserving and sometimes improving sentence-level embedding quality.

\item We analyse the geometry of the word embedding space and find that SALT yields a better-structured cross-lingual representation, improving hubness while preserving isotropy and reducing language-specific clustering.

\end{itemize}

==> SALT/latex/1_intro_old.tex <==
%%%%%%% IGNORE!!


\section{Introduction}
While modern cross-lingual encoders excel at aligning sentences across languages, their behaviour at finer levels of linguistic structure remains largely unexplored. In particular, little is known about whether cross-lingual alignment consistently emerges at the level of phrases and individual tokens.

%Two sentences may share similar representations, even if the words and phrases that compose them are poorly aligned across languages.




-> fer un exemple on hi hagi un poor alignment!!!!! 






. Early research focused on the development of static word embeddings or token representations~\citep{DBLP:conf/nips/BengioDV00, word2vec, glove, fasttext}. 


The advent of Masked Language Modeling (MLM) enabled models to generate contextual word embeddings that capture nuanced meaning based on surrounding text~\citep{bert}. This foundation was extended to the multilingual setting, resulting in models such as M-BERT and XLM that are trained on corpora from multiple languages~\citep{bert, xlm} to facilitate knowledge transfer across languages. This improved performance on cross-lingual tasks, although certain challenges—such as effective alignment of words and handling of low-resource languages remain.

Recent efforts in building strong cross-lingual representations have focus at the \textit{sentence} level~\citep{laser, labse, sonar, mexma, sonar2}. This has advantages for [...]. 

[TOKEN EMBEDDINGS ARE PRACTICALLY IMPORTANT: MTQE, SEQ TAGGING, LABEL EXTRAP.]

However, we a current limitation. 

[WHAT WE DO HERE]

We focus on the three key research questions (RQs): (i) Do sentence embedders preserve local information that is usable for token-rich tasks? (ii) Can additional unsupervised training objective enhance these properties while preserving the sentence-level space? (iii) What are the trade-offs between an improved local (token-level) and global (sentence-level) alignments? 

The key contributions of this work are:
\begin{itemize}
    \item We study token embeddings of sentence representations. 
    \item We study using losses to improve the local representations. We study the trade-offs. 
\end{itemize}

==> SALT/latex/1_intro_oldold.tex <==

%%%%%%% IGNORE!!



\newpage
Multilingual sentence encoders have become a central component of cross-lingual NLP. Models such as SONAR~\citep{sonar} or MEXMA~\citep{mexma} learn a shared embedding space in which semantically equivalent sentences across languages are mapped to nearby representations, achieving strong performance on tasks such as cross-lingual retrieval, sentence mining, and zero-shot classification.

While sentence-level alignment is explicitly optimised during training, these models are often repurposed as token encoders despite never being trained for this setting. This creates a structural mismatch: sentence encoders are supervised to preserve global semantic similarity, yet are widely used in tasks that depend on fine-grained token- and span-level correspondence. As a result, they may produce well-structured sentence embeddings while still exhibiting weak or inconsistent token-level alignment. In practice, many downstream applications rely on token embeddings derived from sentence encoders, including word alignment~\citep{simalign}, sequence tagging~\citep{peters-etal-2017-semi}, hallucination detection~\citep{ottawa} or label projection~\citep{labelproj}.

In this work, we investigate whether the token representations of multilingual sentence encoders can be improved through additional training objectives that operate at a finer granularity. We argue that sentence-level translation data implicitly encodes \textit{span}-level alignment structure that is systematically ignored by standard training objectives.

Our key observation is that translation pairs provide a natural signal not only at the sentence level but also at the lower level of \emph{spans}—contiguous sequences of tokens that express equivalent meaning across languages (see Figure~\ref{diagram}). This signal allows us to directly encourage the alignment of semantically corresponding phrases while maintaining the global structure of the sentence embedding space.

To this end, we propose \salt{0.05} \textbf{SALT} (\textbf{S}pan-\textbf{A}ligned \textbf{L}earning for cross-lingual \textbf{T}okens), a lightweight post-training procedure for multilingual sentence encoders. SALT introduces span-level contrastive and translation objectives to refine token representations, alongside a sentence-level interpolation loss that preserves the original embedding space. Crucially, SALT can be applied to an existing sentence encoder without architectural modifications and is compatible with decoders produced during pre-training.

We evaluate SALT on a suite of multilingual token-level benchmarks, including word alignment, cross-lingual sequence tagging and word sense disambiguation. SALT consistently improves token-level performance while maintaining strong sentence-level representations. In particular, SALT achieves the best overall performance among several alternative fine-tuning strategies on four out of five token-level benchmarks. At the same time, sentence-level evaluation shows that the method preserves--and in some cases improves--the quality of the original embedding space.

Our contributions are the following:

\begin{itemize}
%\item We introduce SALT, a span-aligned post-training method that improves cross-lingual token representations while preserving sentence-level alignment. SALT can use either local or external alignments. 
%\item We demonstrate that our span-level supervision provides a complementary training signal that leads to consistent improvements across multiple multilingual tasks.

\item We propose \textbf{SALT}, a lightweight post-training method that improves cross-lingual token representations via span-aligned objectives.

\item SALT consistently improves performance in multiple token-level multilingual tasks, including word alignment, sequence tagging, and word sense disambiguation, while improving sentence-level performance.

\item SALT is flexible and plug-and-play, supporting both automatically induced (local) and externally provided span alignments, and can be applied to existing sentence encoders and decoders without architectural modifications.
\end{itemize}


==> SALT/latex/2_related_work.tex <==
\section{Related work}

\paragraph{Sentence encoders} Cross-lingual sentence encoders aim to learn a shared semantic space in which sentences with equivalent meaning across languages are mapped to nearby embeddings. Early approaches based on multilingual word embeddings have evolved into large-scale sentence encoders trained on parallel corpora using contrastive, regression, or decoding objectives. Models such as SONAR~\citep{sonar}, MEXMA~\citep{mexma}, OmniSONAR~\citep{sonar2} or LaBSE~\citep{labse} exemplify this paradigm. 

%\paragraph{Word and phrase alignment} Early statistical machine translation relied on word alignment models and derived phrase pairs from these alignments as translation units~\citep{DBLP:journals/coling/BrownPPM94, DBLP:conf/naacl/KoehnOM03}. More recently, word alignment has been revisited in the context of neural encoders, with methods designed to extract alignments directly from contextual representations~\citep{simalign}. A related line of work improves the alignment properties of cross-lingual encoders through fine-tuning objectives that encourage better token-level correspondence across languages~\citep{chi-etal-2021-improving, DBLP:conf/eacl/DouN21}.

\paragraph{Word and phrase alignment}
Early statistical machine translation relied on word alignment models and derived phrase pairs as discrete translation units for decoding~\citep{DBLP:journals/coling/BrownPPM94, DBLP:conf/naacl/KoehnOM03}, establishing a notion of cross-lingual span correspondence. While this is related in spirit to SALT, we use such span correspondences only as a training signal. More recently, word alignment has been revisited in neural encoders, with methods extracting alignments from contextual representations~\citep{simalign}. Related work improves cross-lingual alignment through objectives that encourage finer-grained token-level correspondence~\citep{chi-etal-2021-improving, DBLP:conf/eacl/DouN21}.
\paragraph{Bridging sentence- and token-level representations}
Prior work improves cross-lingual sentence encoders by incorporating auxiliary word- or token-level objectives during pre-training~\citep{DBLP:conf/iclr/WeiW0XYL21, alqahtani-etal-2021-using-optimal, li-etal-2021-multi, dap, miao-etal-2024-enhancing}, typically relying on explicit alignment signals to enhance sentence-level embeddings. In contrast, we directly target token- and span-level representations, both in training and evaluation, explicitly focusing on improving their quality rather than treating them as a by-product of sentence-level learning, focusing on adapting existing sentence encoders for token-centric tasks.

%Closest to our work, \citet{sonar2} propose OmniSONAR-Token, a word-alignment-based intervention; SALT yields stronger token-level representations by leveraging span-level supervision.   

%%% DO I CITE VECO 2.0 (not published) https://arxiv.org/pdf/2304.08205 



==> SALT/latex/3_method.tex <==
\section{\salt{0.05} SALT: Span-Aligned Learning for Cross-Lingual Tokens}
To improve cross-lingual token representations produced by sentence encoders, we propose SALT, a training method that aligns semantically equivalent spans across languages. SALT is lightweight and can be applied post-training to any pre-trained encoder without modifying its architecture.
As illustrated in Figure~\ref{diagram}, we first extract semantically equivalent multi-word spans from parallel sentences and precompute their corresponding sentence representations. During training, span-level alignment objectives refine token and span embeddings while preserving the structure of the original sentence-level representation space.

\subsection{Method} Let $x$ and $y$ be a translation pair. A tokeniser $\mathcal{T}$ with vocabulary $V$ maps them to token sequences $t_x=\mathcal{T} (x) \in V^n$ and $t_y=\mathcal{T} (y) \in V^m$. A pretrained encoder $\mathcal{E}$ then produces contextual embeddings $H_x = \mathcal{E}(t_x) \in \mathbb{R}^{n \times d}$ and $H_y = \mathcal{E}(t_y) \in \mathbb{R}^{m \times d}$. These representations are typically trained such that their pooled sentence embeddings are aligned, i.e., $\text{pool}(H_x) \approx \text{pool}(H_y)$. Following \citet{sonar}, we adopt average pooling, although our approach is compatible with alternative strategies, such as max pooling or the use of a designated [CLS] token (as in \citet{mexma}).

We define a \textit{span pair} as a pair of contiguous token subsequences from a translation pair with similar contextual meaning. Formally, it is given by $(t_x[i:j], t_y[i':j'])$. $t_x[i:j]$ denotes tokens $i,\dots,j−1$ with \(0\le i<j\le n;\;0\le i'<j'<m\). The span representations are obtained by pooling the token embeddings within each subsequence, i.e., $\text{pool}(H_x[i:j])$ and $\text{pool}(H_y[i':j'])$. 

\subsubsection{Span extraction}
We require aligned spans across parallel sentences to construct training supervision. We consider two approaches for span extraction: (i) an LLM-based method, and (ii) a lightweight heuristic, CASE.

In most of our experiments, we use LLaMA-70B~\citep{DBLP:journals/corr/abs-2407-21783} to extract aligned spans (see Appendix~\ref{span:extraction}). However, LLM-based extraction can be computationally expensive and not always available. To address this, we introduce CASE (Constituent Alignment Span Extraction), a heuristic that extracts aligned spans using token-level alignments derived from encoder $\mathcal{E}$ representations. %(Algorithm~\ref{case}).

\paragraph{CASE}
Given a source sentence $x$, we compute token-level alignments $M: \{0, \dots, n-1\} \rightarrow \{0, \dots, m-1\} \cup \{\varnothing\}$ using Argmax~\citep{simalign}, extended to multi-token words. For a target token $t$, we define the inverse mapping $M^{-1}(t) = \{ s \mid M(s) = t\}$.

We consider candidate source spans $t_x[i:j]$. Let $A_{i:j} = \{ M(s) \mid s \in \{i, \dots, j-1\},\; M(s) \neq \varnothing \}$. Then we define the aligned target span as the tightest span covering all aligned tokens:
$i' = \min A_{i:j}$, \;
$j' = \max A_{i:j} + 1$. To ensure syntactic validity, we restrict source spans to constituents identified using the Benepar parser~\citep{DBLP:conf/acl/KitaevCK19}. We discard span pairs for which alignment links are not fully contained within the span pair, i.e., no token in the target span is aligned to a source token outside the source span, and vice versa.

Finally, we define the coverage of a span pair as the proportion of aligned tokens in both directions:
\begin{equation}
\begin{small}
\begin{aligned}
\mathrm{cover} &= \frac{\mid\{s \mid s \in \{i, \dots, j-1\}, M(s) \neq \varnothing \}\mid}{2((j - i)+(j' - i'))}  \\
    &+ \frac{\mid\{t  \mid  t \in \{i', \dots, j'-1\}, M^{-1}(t) \neq \varnothing \}\mid}{2((j - i)+(j' - i'))}
\end{aligned}
\end{small}
\end{equation}

We discard any pair of source-target spans whose coverage falls below a threshold $c$ = 0.7, ensuring that only well-aligned spans are used. %A high coverage value indicates that most tokens in both spans are mutually aligned, while a low value indicates poor alignment. 

\paragraph{Evaluation of span extraction}
We evaluate span quality via human evaluation on Chinese (\texttt{zho\_Hans}), French, Hindi, Russian, and Spanish. Spans are extracted from English–target sentence pairs from our word alignment dataset (Section~\ref{token_eval}). We recruit 7 native speakers to annotate a total of 2,361 span pairs for both LLaMA-70B and CASE (with SONAR), rating span semantic equivalence on a 4-point scale: (1) unrelated, (2) somewhat related, (3) nearly equivalent, (4) equivalent. See Appendix~\ref{annotation} for guidelines and full results.

Figure~\ref{human_eval} shows the score distribution. Both LLaMA-based extraction and CASE yield high-quality span pairs, with over 90\% of annotations in the top two categories. LLaMA performs better on Russian and French, while CASE matches or exceeds it in other languages. We retain score-4 spans to construct CrossSpan for the evaluation in Section~\ref{analysis_sec}. Overall, both methods effectively identify semantically equivalent spans, supporting their use as supervision signals. CASE offers an efficient alternative to LLM-based extraction while preserving alignment quality.




\begin{figure}
  \centering
  %left bottom right top
\includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=\columnwidth]{latex/figs/rating_distribution_grouped_bars_4_langs.pdf}
    \caption{Human evaluation of extracted spans. Score distributions for LLaMA-70B and SONAR (CASE). }
    \label{human_eval}
    \vspace{-5pt}
\end{figure}


\subsubsection{SALT training objective} SALT uses a translation (MT) and a contrastive (CON) objective at the span level, as well as an interpolation objective (INT) at the sentence level.

\begin{equation}
    \mathcal{L}_{SALT} =  \mathcal{L}_{CON_{Span}} + \alpha \mathcal{L}_{MT_{Span}} + \beta \mathcal{L}_{INT} 
\end{equation}
where $\alpha, \beta \in \mathbb{R}$ are hyperparameters set to one unless otherwise specified. For simplicity, we present the losses for a single translation pair $(x, y)$, though they are computed in batches during training.
\paragraph{Contrastive objective} 
We apply the span extraction method (LLM or CASE) to obtain a collection of $p$ aligned spans 
$t_x[i^1: j^1], \dots, t_x[i^p: j^p]$ and $t_y[i'^1: j'^1],\dots, t_y[i'^p: j'^p]$.

To increase coverage of both sentences, we augment this set with unaligned spans. Specifically, for every maximal contiguous subsequence of tokens that does not belong to any aligned span, we form an additional span. This yields additional spans $(t_x[i^{p+1}: j^{p+1}], \dots, t_x[i^{q}: j^{q}])$ and $(t_y[i'^{p+1}: j'^{p+1}], \dots, t_y[i'^{v}: j'^{v}])$.

We compute the corresponding span embeddings $H_x^1,\dots,H_x^q$ and $H_y^1,\dots,H_y^v$ by averaging the token embeddings within each span. We then define the contrastive loss as

\begin{equation}
\begin{small}
\begin{aligned}
 \mathcal{L}_{\text{CON}_{Span}} 
 &= -\frac{1}{p} \sum_{i=1}^{p} \Bigg[
\log
\frac{\exp(\langle H_x^i, H_y^i \rangle / \tau)}
{\sum_{j=1}^{v} \exp(\langle H_x^i, H_y^j \rangle / \tau)}
\\
&\qquad +
\log
\frac{\exp(\langle H_x^i, H_y^i \rangle / \tau)}
{\sum_{j=1}^{q} \exp(\langle H_x^j, H_y^i \rangle / \tau)}
\Bigg]
\end{aligned}
\end{small}
\end{equation}

where $\langle \cdot, \cdot \rangle$ denotes the dot product, $(H_x^i, H_y^i)$ corresponds to an aligned span pair, and $\tau$ is a temperature hyperparameter. The first term applies a row-wise softmax over target spans for each source span, while the second term applies a column-wise softmax over source spans for each target span. This loss encourages semantically equivalent spans to have similar embeddings while pushing apart spans with different meanings.

\paragraph{Translation objective} 
Given a pre-trained decoder $\mathcal{D}$ that we keep frozen, we define the translation loss as the cross-entropy over the target span:
\begin{equation}
\begin{small}
\mathcal{L}_{\text{MT}_{\text{Span}}} \! = \! -\tfrac{1}{p}\sum_{l=1}^{p} \sum_{k=i'^l}^{j'^l\!-\!1}\! \log P_\mathcal{D}\big(t_y[k] ; t_y[i'^l:k] , H_x^l\big)
\end{small}
\end{equation}
where ($t_x[i^l:j^l]$ and $t_y[i'^l:j'^l]$) is an extracted span pair, $H_x^l$ is the pooled source span representation and $P_\mathcal{D}$ denotes the probability assigned by the decoder to the next target token, conditioned on the previous target tokens and the pooled representation of the source span. 

\paragraph{Interpolation objective} 
Following~\citet{DBLP:conf/acl/TsiamasDC25}, we introduce a sentence-level interpolation objective that encourages the encoder to preserve the original sentence representation space. We obtain a teacher representation $z_{xy}$ by averaging the source and target sentence embeddings produced by the frozen encoder $\mathcal{E}^{frozen}$. The interpolation loss is then defined as

\begin{equation}
\small 
   \mathcal{L}_{INT} = \text{MSE}\Big(z_{xy}, \text{pool}(H_x)\Big) + \text{MSE}\Big(z_{xy}, \text{pool}(H_y)\Big)
\end{equation}

where $\text{MSE}$ denotes the mean squared error. Intuitively, this loss constrains the encoder so that token-level training objectives do not distort the sentence-level embedding space, maintaining consistency with the initial frozen encoder.




==> SALT/latex/4_experiments.tex <==
\begin{table}[hbtp!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc}
\toprule

\bf{\makecell{Task \\ (\#langs)}}& \textbf{Example} \\
\midrule
\makecell{AER\\(18)} &

\raisebox{-0.5\height}{%
\begin{tikzpicture}[
  every node/.style={inner sep=1pt, outer sep=0pt}
]

% English
\node[anchor=base] (en1) at (0,0) {The};
\node[anchor=base] (en2) at ([xshift=8.1mm] en1.base east) {necessary};
\node[anchor=base] (en3) at ([xshift=9.1mm] en2.base east) {correction};
\node[anchor=base] (en4) at ([xshift=4.1mm] en3.base east) {will};
\node[anchor=base] (en5) at ([xshift=3.1mm] en4.base east) {be};
\node[anchor=base] (en6) at ([xshift=6.1mm] en5.base east) {made};
\node[anchor=base] (en7) at ([xshift=2.1mm] en6.base east) {.};

% German
\node[anchor=base west] (de1) at ([yshift=-10mm] en1.base west) {Eine};
\node[anchor=base] (de2) at ([xshift=12mm] de1.base east) {entsprechende};
\node[anchor=base] (de3) at ([xshift=8.1mm] de2.base east) {Anderung};
\node[anchor=base] (de4) at ([xshift=4.1mm] de3.base east) {wird};
\node[anchor=base] (de5) at ([xshift=11mm] de4.base east) {vorgenommen};
\node[anchor=base] (de6) at ([xshift=6.1mm] de5.base east) {werden};
\node[anchor=base] (de7) at ([xshift=4.1mm] de6.base east) {.};

% Links
\draw[<->,thick] (de1.north) -- (en1.south);
\draw[<->,thick] (de2.north) -- (en2.south);
\draw[<->,thick] (de3.north) -- (en3.south);
\draw[<->,thick] (de4.north) -- (en4.south);
\draw[<->,thick] (de5.north) -- (en6.south);
\draw[<->,thick] (de6.north) -- (en5.south);
\draw[<->,thick] (de7.north) -- (en7.south);

\end{tikzpicture}%
}
\\
\addlinespace[8pt]

\makecell{Massive\\(52)} &
\begin{tabular}[c]{@{}l@{}}
What is today 's forecast for Berlin\\
        \makebox[0pt][l]{\hspace{3.7em}\footnotesize DATE}%
        \makebox[0pt][l]{\hspace{11.7em}\footnotesize	 PLACE}%
\end{tabular}
\\
\addlinespace[8pt]

\makecell{PAN-X\\(40)} &
\begin{tabular}[c]{@{}l@{}}
REDIRECCIÓN Algarrobo ( Chile ) \\

        \makebox[0pt][l]{\hspace{8.3em}\footnotesize B-LOC}%
        \makebox[0pt][l]{\hspace{12em}\footnotesize	 I-LOC}%


\end{tabular}
\\
\addlinespace[8pt]

\makecell{UDPOS\\(51)} &
\begin{tabular}[c]{@{}l@{}}
\foreignlanguage{japanese}{葬儀\hspace{1.3em}の\hspace{1.3em}最中\hspace{1.3em}です\hspace{1.2em}よ\hspace{1.8em}!}  \\

        \makebox[0pt][l]{\hspace{0em}\footnotesize NOUN}%
        \makebox[0pt][l]{\hspace{3.1em}\footnotesize	 ADP}%
        \makebox[0pt][l]{\hspace{5.5em}\footnotesize	 NOUN}%
        \makebox[0pt][l]{\hspace{9.0em}\footnotesize	 AUX}%
        \makebox[0pt][l]{\hspace{11.6em}\footnotesize	 PART}%
        \makebox[0pt][l]{\hspace{14em}\footnotesize	 PUNCT}%


\end{tabular}
\\
\addlinespace[8pt]


\makecell{WiC \\(6)} &
\begin{tabular}[c]{@{}l@{}}
$\left.
\begin{array}{@{}l@{}}
\text{Bolivia holds a key \underline{play} in this process of peace.} \\
\text{A musical \underline{play} on the same subject was also staged.}
\end{array}
\right\}\ 
\begin{array}{@{}l@{}}
\text{Different}\\
\text{meaning}
\end{array}$
\end{tabular}
\\
\bottomrule
\end{tabular}}
\caption{Summary of the tasks and number of languages used for the evaluation of cross-lingual token representations. Source: \citet{sonar2}}
%This table is an adaptation from~\citet{sonar2}.
\label{example_datasets}
\vspace{-5pt}
\end{table}


\section{Experiment details}
We initialise $\mathcal{E}$,$\mathcal{D}$ with the respective pre-trained SONAR weights~\citep{sonar}.


\paragraph{Data} We fine-tune SONAR on a subset of the data originally used to train it, namely the publicly available NLLB Primary dataset~\citep{DBLP:journals/corr/abs-2207-04672}.~\footnote{Downloaded using the script provided at \href{https://github.com/gordicaleksa/Open-NLLB/blob/nllb_replication/examples/nllb/data/README.md}{https://github.com/gordicaleksa/Open-NLLB}.}
 This dataset comprises high-quality parallel sentences spanning a diverse set of languages. We begin by excluding all language pairs for which neither language belongs to the set of 57 designated test languages, yielding a total of 129 language pairs (see Appendix~\ref{langs_info}). The 29 test languages not observed during training can be used to evaluate the generalisation of our method (see Appendix~\ref{test_unseen_bruto}). 

For each retained language pair, we downsample the corpus to 40{,}000 sentence pairs, observing no degradation in performance as a result of this reduction. In line with the procedure of~\citet{sonar2}, we further refine the dataset by removing sentence pairs whose BLASER 2 score~\citep{DBLP:conf/emnlp/DaleC24} deviates by more than one standard deviation from the mean score computed for the given language pair.

\paragraph{Training hyperparameters} We train SONAR for 20,000 steps, with a maximum of 1400 tokens per batch (roughly corresponding to 50 pairs of sentences per batch) and a learning rate of $\mu=10e-5$. We use an AdamW optimiser~\citep{DBLP:conf/iclr/LoshchilovH19} and warm-up of 1000 steps. We do the training runs on three seeds and report average values in all experiments unless otherwise specified. Standard deviations are reported in Appendix~\ref{stdev}.

\paragraph{Baselines} We report the performance of the encoders XLM-R~\citep{xlm}, XLM-Align~\citep{chi-etal-2021-improving}, LaBSE~\citep{labse}, and MEXMA~\citep{mexma}. In addition, we compare SALT against variants obtained by fine-tuning SONAR with alternative training objectives. Specifically, we train the encoder for longer using the original SONAR loss proposed by~\citet{sonar}. We also include token-level objectives: the Self-Objective (SO) loss~\citep{DBLP:conf/eacl/DouN21}, a contrastive word-alignment objective; the WordOT loss~\citep{alqahtani-etal-2021-using-optimal}, using Optimal Transport; the WACSE loss~\citep{miao-etal-2024-enhancing}, which adds a masked language modeling head; and the OmniSONAR-Token loss~\citep{sonar2}, which extends SO loss with interpolation. See Appendix~\ref{losses:implement} for implementation details.

\paragraph{Sentence evaluation} We evaluate the task of sentence mining using the FLORES-200 devtest~\citep{nllb} (80 languages) and report xsim~\citep{labse} and xsim++~\citep{xsimplusplus}. For classification, we report on tasks from MTEB~\citep{muennighoff-etal-2023-mteb} (English only). 

\subsection{Cross-lingual token evaluation}
\label{token_eval}
Standard benchmarks often evaluate sentence encoders through sequence-level tasks, which can mask weaknesses in token representations~\citep{conneau2018xnli, xtreme, DBLP:conf/iclr/EnevoldsenCKKMS25}. Following~\citet{sonar2}, we instead focus on tasks that isolate the embeddings of individual tokens, providing a more rigorous assessment of cross-lingual token quality. For word alignment, we test whether tokens across languages align semantically. For sequence tagging, we feed the classifier head only the embedding of a single word to directly probe the quality of its token-level representations across languages.

\paragraph{Word alignment} Given a translation pair $x, y$, the task of word alignment identifies which words correspond to each other semantically. More formally, given a source–target sentence pair $x$, $y$ with word lengths $w_x$, $w_y$, respectively, we infer a binary matrix $M\in\{0,1\}^{w_s \times w_y}$, where $M_{ij}=1$ represents that the $i$-th word in the source sentence aligns semantically with the $j$-th word in the target sentence. We present an example in Table~\ref{example_datasets}.

Many current word alignment methods derive alignments based on the similarity of token embeddings~\citep{simalign, DBLP:conf/acl/AzadiFD23}. We define the \textit{token similarity matrix} $S\in \mathbb{R}^{n\times m}$; $S_{i,j}:=sim(\mathcal{E}(t_x[i]), \mathcal{E}(t_y[j]))$, where \textit{sim} is a similarity measure (we use cosine similarity), $t_x[i]$ and $t_y[j] \in V$ are the $i$-th and $j$-th tokens of the source and target sentences $x$ and $y$. An \textit{extraction} method is then applied to convert these similarities into a discrete alignment. We use Itermax~\citep{simalign} to extract alignments and report Alignment Error Rate (AER)~\citep{DBLP:conf/acl/OchN00}. The full list of alignment datasets is in Appendix~\ref{alignment_datasets}. 



%\paragraph{Sequence tagging} Given an input sequence of tokens $x = (x_1, x_2, \dots, x_n)$, the goal is to assign a label $y_i \in \{1, \dots, N \}$ to each token $x_i$. To test how well different encoders learn cross-lingual token representations, we train a classifier head $C\in \mathbb{R}^{d \times N}$ on top of the encoder embeddings, thus keeping the encoder frozen. The head is trained only on English data and then evaluated zero-shot on all available languages.

%We report performance for the following datasets: Massive (slot filling)~\citep{fitzgerald2022massive}, PAN-X (Named Entity Recognition)~\citep{DBLP:conf/acl/PanZMNKJ17}, UDPOS (Part of Speech)~\citep{DBLP:conf/lrec/NivreMGHMPSTZ20} and WiC (word sense disambiguation)~\citep{DBLP:conf/naacl/PilehvarC19}. For WiC, which is not a sequence tagging task, we adapt the evaluation as follows: we extract the contextual representation of the target word in each sentence, concatenate the two vectors, and apply a classifier head $C\in \mathbb{R}^{2d \times 2}$. For multi-token targets, we obtain the word representation by averaging the representations of its subword tokens.

%When the dataset segmentation does not perfectly align with the tokeniser (e.g., a token overlaps with multiple segments assigned to different classes), we assign the token the label of the segment with the largest character-level overlap. If there is a tie, we assign the label of the earliest overlapping segment.

\paragraph{Sequence tagging}
We evaluate token-level cross-lingual representations using standard sequence labelling tasks, where each token $x_i$ in an input sequence $x = (x_1, \dots, x_n)$ is assigned a discrete label $\{1, \dots, N\}$. To isolate the contribution of the encoder, we train a linear classification head $C \in \mathbb{R}^{d \times N}$ placed on top of the token embeddings while keeping the encoder parameters fixed. The classifier is trained only on English data and subsequently evaluated in other languages (zero-shot); see Appendix~\ref{seq:implement} for implementation details. 

We consider a diverse set of benchmarks, including Massive (Slot Filling)~\citep{fitzgerald2022massive}, PAN-X (Named Entity Recognition)~\citep{DBLP:conf/acl/PanZMNKJ17}, UDPOS (Part-of-Speech Tagging)~\citep{DBLP:conf/lrec/NivreMGHMPSTZ20}, and WiC (Word Sense Disambiguation)~\citep{DBLP:conf/naacl/PilehvarC19}. WiC is not technically a sequence tagging task; we adapt it by extracting the contextual embeddings of the target word in each sentence, concatenating the resulting vectors, and feeding them into a classifier $C \in \mathbb{R}^{2d \times 2}$. When a target word is split into multiple subword tokens, we represent it by averaging the corresponding embeddings.

Finally, to handle mismatches between dataset annotations and tokeniser segmentation, we map labels to tokens based on maximal character overlap. When multiple segments overlap a token equally, we resolve ties by selecting the first.

==> SALT/latex/4_experiments_old.tex <==
Table~\ref{alignment}
Table~\ref{best_layer}

\begin{table*}[]
\centering
{\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
                   & \textbf{Average}   & \textbf{de-en} & \textbf{en-bg} & \textbf{en-cs} & \textbf{en-da} & \textbf{en-es} & \textbf{en-et} & \textbf{en-fa} & \textbf{en-fr} & \textbf{en-hi} & \textbf{en-hu} & \textbf{en-it} & \textbf{en-nl} & \textbf{en-pt} & \textbf{en-ru} & \textbf{en-sl} & \textbf{ja-en} & \textbf{ro-en} & \textbf{zh-en} \\
                   \midrule
\footnotesize XLM-Roberta & 0.203          & 0.192          & 0.147          & 0.126          & 0.093          & 0.144          & 0.195          & 0.308          & 0.064          & 0.379          & 0.214          & 0.189          & 0.072          & 0.149          & 0.147          & 0.185          & 0.503          & 0.258          & 0.288          \\
\footnotesize XLM-v       & 0.206          & 0.188          & 0.146          & 0.123          & 0.102          & 0.137          & 0.184          & 0.311          & 0.063          & 0.383          & 0.208          & 0.185          & 0.067          & 0.143          & 0.156          & 0.18           & 0.532          & 0.268          & 0.326          \\
\footnotesize XLM-Align   & 0.184          & 0.167          & 0.13           & 0.106          & 0.085          & 0.129          & 0.185          & 0.289          & 0.056          & 0.328          & 0.205          & 0.17           & 0.062          & 0.135          & 0.134          & 0.176          & 0.455          & 0.253          & 0.242          \\
\footnotesize MEXMA              & \textbf{0.166} & \textbf{0.163} & \textbf{0.124} & \textbf{0.091} & \textbf{0.074} & \textbf{0.119} & \textbf{0.148} & \textbf{0.251} & \textbf{0.047} & \textbf{0.292} & \textbf{0.193} & \textbf{0.163} & \textbf{0.05}  & \textbf{0.131} & \textbf{0.126} & 0.161          & \textbf{0.428} & 0.217          & 0.212          \\
\footnotesize SONARv1            & 0.174          & 0.184          & 0.131          & 0.095          & 0.081          & 0.123          & 0.159          & 0.268          & 0.054          & 0.3            & 0.206          & 0.174          & 0.065          & 0.136          & 0.129          & \textbf{0.158} & 0.441          & \textbf{0.216} & \textbf{0.207} \\
\footnotesize SONARv2            & 0.19           & 0.207          & 0.14           & 0.119          & 0.089          & 0.144          & 0.166          & 0.297          & 0.071          & 0.326          & 0.216          & 0.19           & 0.074          & 0.143          & 0.148          & 0.185          & 0.443          & 0.251          & 0.22           \\
\footnotesize SONAR-Omni         & 0.192          & 0.207          & 0.138          & 0.114          & 0.094          & 0.144          & 0.167          & 0.307          & 0.071          & 0.315          & 0.221          & 0.187          & 0.072          & 0.14           & 0.152          & 0.185          & 0.449          & 0.256          & 0.23          
\\
\bottomrule
\end{tabular}}
\caption{AER for }
\label{alignment}
\end{table*}


\begin{table}[]
\centering
{
\begin{tabular}{lcc}
\toprule
                   & \multicolumn{1}{l}{Best} & \multicolumn{1}{l}{Average} \\
                   \midrule
XLM-Roberta & 8                              & 0.203                \\
XLM-v      & 7                              & 0.201                   \\
XLM-Align & 8                              & 0.184                   \\
MEXMA              & 20                             & 0.163                   \\
SONARv1            & 19                             & 0.161                   \\
SONARv2            & 8                              & 0.165                   \\
SONAR-Omni         & 8                              & 0.167                  \\
\bottomrule
\end{tabular} }
\caption{AER for }
\label{best_layer}
\end{table}





\subsection{Sequence tagging}
Table~\ref{seq:label}
\begin{table*}[]
\centering
{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccccc}
\toprule
& \shortstack{Massive \\ {\small (English)}}
& \shortstack{Massive \\ {\small (All)}}
& \shortstack{Massive \\ {\small (Single)}}
& \shortstack{PAN-X \\ {\small (English)}}
& \shortstack{PAN-X \\ {\small (All)}} & \shortstack{PAN-X \\ {\small (Single)}}
& \shortstack{UDPOS \\ {\small (English)}}
& \shortstack{UDPOS \\ {\small (All)}} & \shortstack{UDPOS \\ {\small (Single)}}\\
\midrule
mBERT       & 0.142                                                                                          & 0.306                                                                                      & 0.458                & 0.576                                                                                        & 0.695                                                                                    & 0.812                & 0.426                                                                                        & 0.565                                                                                    & 0.718                \\
XLM-Roberta & 0.230                                                                                          & 0.410                                                                                      & 0.468                & 0.546                                                                                        & 0.640                                                                                    & 0.762                & 0.507                                                                                        & 0.617                                                                                    & 0.763                \\
XLM-v       & 0.269                                                                                          & 0.480                                                                                      & 0.495                & 0.594                                                                                        & 0.692                                                                                    & 0.786                & \textbf{0.528}                                                                               & \textbf{0.634}                                                                           & 0.755                \\
MEXMA       & 0.454                                                                                          & 0.599                                                                                      & \textbf{0.573}       & 0.611                                                                                        & 0.708                                                                                    & \textbf{0.819}                & 0.522                                                                                        & 0.593                                                                                    & \textbf{0.764}       \\
SONARv1     & 0.446                                                                                          & 0.574                                                                                      & 0.561                & 0.594                                                                                        & 0.698                                                                                    & 0.805                & 0.522                                                                                        & 0.565                                                                                    & 0.720                \\
SONARv2     & \textbf{0.490}                                                                                 & 0.602                                                                                      & 0.567                & 0.616                                                                                        & \textbf{0.716}                                                                           & 0.817       & 0.519                                                                                        & 0.585                                                                                    & 0.750                \\
SONAR-Omni  & 0.479                                                                                          & \textbf{0.607}                                                                             & 0.567                & \textbf{0.624}                                                                               & 0.710                                                                                    & 0.809                & 0.520                                                                                        & 0.580                                                                                    & 0.725                \\ 
\bottomrule                   
\end{tabular} }
\caption{blabla}
\label{seq:label}
\end{table*}





\begin{table*}[]
\centering
{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
& \shortstack{Massive \\ {\small (English)}}
& \shortstack{Massive \\ {\small (All)}}
& \shortstack{PAN-X \\ {\small (English)}}
& \shortstack{PAN-X \\ {\small (All)}}
& \shortstack{UDPOS \\ {\small (English)}}
& \shortstack{UDPOS \\ {\small (All)}} \\
\midrule
MEXMA            & 0.454                                                                                          & 0.599                                                                                      & 0.611                                                                                        & 0.708                                                                                    & 0.522                                                                                        & 0.593                                                                                    \\
SONARv1 (frozen) & 0.446                                                                                          & 0.574                                                                                      & 0.594                                                                                        & 0.698                                                                                    & 0.522                                                                                        & 0.565                                                                                    \\
Teacher Loss     & 0.478                                                                                          & 0.589                                                                                      & 0.606                                                                                        & 0.711                                                                                    & 0.502                                                                                        & 0.561                                                                                    \\
SO (R=0.3)       & 0.461                                                                                          & 0.586                                                                                      & 0.607                                                                                        & 0.709                                                                                    & 0.527                                                                                        & 0.577                                                                                    \\
SONARv2          & \textbf{0.490}                                                                                 & 0.602                                                                                      & 0.616                                                                                        & \textbf{0.716}                                                                           & 0.519                                                                                        & 0.585                                                                                    \\
SONAR-Omni       & 0.479                                                                                          & \textbf{0.607}                                                                             & \textbf{0.624}                                                                               & 0.710                                                                                    & 0.520                                                                                        & 0.580                                                                                    \\
\bottomrule                   
\end{tabular} }
\caption{blabla}
\label{seq:label}
\end{table*}




\subsection{Machine Translation Quality Estimation}

==> SALT/latex/5_results.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
                & \textbf{AER ($\downarrow$)} & \textbf{PAN-X ($\uparrow$)}          & \textbf{Massive ($\uparrow$)}        & \textbf{UDPOS ($\uparrow$)}          & \textbf{WiC ($\uparrow$)}\\
\midrule
\textit{Pre-trained encoders} \\
XLM-R     & 0.307                                           & 0.551          & 0.220          & 0.527          & 0.538          \\
XLM-Align       & 0.246                                                & 0.532          & 0.187          & 0.522          & 0.556          \\
LaBSE           & 0.232                                      & 0.589          & 0.431          & 0.551          & 0.538          \\
%$m5E_{large}$  & 0.332                                            & 0.499          & 0.256          & 0.411          & 0.543          \\
MEXMA           & \textbf{0.171}                            & 0.593          & 0.396          & 0.553          & 0.565          \\
%DAP             & 0.204                                         & 0.527          & 0.376          & 0.528          & 0.575          \\
SONAR           & 0.183                                         & 0.582          & 0.402          & 0.548          & 0.576          \\

\midrule
\textit{SONAR + additional objectives}
\\
SONAR Loss~\tiny{\citep{sonar}}     & 0.179                                             & 0.588          & 0.426          & 0.554          & 0.581          \\
SO Loss~{\tiny\citep{DBLP:conf/eacl/DouN21}}         & 0.178                                         & 0.597          & 0.410          & \textbf{0.577} & 0.574          \\

WordOT~{\tiny\citep{alqahtani-etal-2021-using-optimal}}  & 0.320 &      0.609    &     0.417      & 0.561  & \textbf{0.585}          \\

WACSE~{\tiny\citep{miao-etal-2024-enhancing}}  & 0.205                                         & 0.600          & 0.409          & 0.569 & 0.573          \\

OmniSONAR-Token~\tiny{\citep{sonar2}} & 0.180                                           & 0.610          & 0.417          & 0.574    & 0.583          \\
SALT \salt{0.05} (ours)          & \textbf{0.171}                            & \textbf{0.622} & \textbf{0.452} & 0.571          & \textbf{0.585} \\
\bottomrule
\end{tabular}}
\caption{Cross-lingual token-level evaluation across five benchmarks for frozen pre-trained encoders and SONAR trained with additional objectives. SALT achieves the best or joint-best performance on four of five benchmarks.}
\label{main-results}
\vspace{-5pt}
\end{table*}


\begin{figure*}[t]
  \centering
  %left bottom right top
\includegraphics[trim={0cm 0.4cm 0cm 0cm},clip, width=1\textwidth]{latex/figs/flores_word_embedding_pca_lang.pdf}
    \caption{Principal component projections of token embeddings for the same sentence across 80 languages. Each colour corresponds to a language. SONAR produces a more distributed and language-agnostic embedding space. Sentence: \textit{The great pyramid was created to honor the Pharaoh Khufu, and many of the smaller pyramids, tombs, and temples were built to honor Khufu's wives and family members.}}
    \label{pca}
    \vspace{-7pt}
\end{figure*}

\section{Results}
Table~\ref{main-results} compares SALT with pre-trained encoders and alternative fine-tuning objectives for SONAR across five cross-lingual token benchmarks. Among the pre-trained models, MEXMA achieves the lowest AER (0.171), while SONAR remains competitive on the other tasks. Continued training with the SONAR loss improves all token-level results, suggesting that SONAR was primarily optimised for sentence mining rather than token representations.

Among the fine-tuning objectives, SALT outperforms in word alignment (AER), PAN-X, Massive, and WiC, showing that span-level objectives provide complementary signals beyond sentence- or token-level training. Gains are particularly pronounced on tasks requiring rich cross-lingual semantics (PAN-X, Massive) and on word alignment. On UDPOS, SALT achieves a strong score of 0.571 (vs. 0.548 for the pre-trained model), but is slightly outperformed by SO Loss (0.577). This may be due to UDPOS being more language-specific, exhibiting limited cross-lingual transfer relative to other tasks (see Appendix~\ref{seq_tagging_udpos})

%This may be due to SO Loss inducing positional encoding effects (see Appendix~\ref{pos-encoding}), which can benefit word-order-sensitive tasks.

Taken together, the results show that SALT achieves the best overall performance among the considered strategies, and suggest that incorporating span-level supervision is an effective and principled way to enrich multilingual sentence representations beyond sentence-level objectives alone.

Does improved token-level representation come at the cost of sentence-level quality? For cross-lingual sentence mining, SALT consistently improves over SONAR on xsim and xsim++ (Table~\ref{tab:merged-eval}). For MTEB classification tasks, SALT matches SONAR on XNLI and MIntent and improves on STS17. Overall, SALT does not sacrifice sentence-level quality and, in several cases, improves it.

%\begin{table}[]
%\centering
%\begin{tabular}{lcc}
%\toprule
%& \multicolumn{2}{c}{\bf \small FLORES (57)} \\
 %     & \small \textbf{xsim ($\downarrow$)} & \small \textbf{xsim ++ ($\downarrow$)} \\
%      \midrule
%\small SONAR & \small 0.2           & \small 9.9                                \\
%\small SALT  & \small \textbf{0.1}  & \small \textbf{9.1}    \\          
%\bottomrule
%\end{tabular}
%\caption{Performance for cross-lingual sentence mining. We report xsim~\citep{laser} and xsim++~\citep{xsimplusplus}.}
%\label{xsim-results}
%\end{table}


%\begin{table}[]
%\centering
%\setlength{\tabcolsep}{3pt}
%\begin{tabular}{lcccc}
%\toprule
%      & \small \textbf{XNLI} & \small \textbf{STS17} & \small \textbf{MScenario} & \small \textbf{MIntent} \\
%      \midrule
%\small SONAR & \small 0.61          & \small 0.65           & \small \textbf{0.64}                                & \small \textbf{0.58}                              \\
%\small SALT  & \small 0.61          & \small \textbf{0.69}  & \small 0.63                                         & \small 0.57        \\
%\bottomrule
%\end{tabular}
%\caption{Accuracy (?) for MTEB classification tasks. We only evaluate English.}
%\label{sentence-class}
%\end{table}




\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{lccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Mining ($\downarrow$) }} & \multicolumn{3}{c}{\textbf{Classification ($\uparrow$)}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6}
& \textbf{xsim} & \textbf{xsim++} 
& \textbf{XNLI}  & \textbf{STS17} & \textbf{MIntent} \\
\midrule
\small SONAR & \small 0.2 & \small 9.9 & \small 0.61 & \small 0.65 & \small 0.58 \\
%\small SALT  & \small \textbf{0.1} & \small \textbf{9.1} & \small 0.61 & \small \textbf{0.69} & \small 0.57 \\
\small SALT  & \small \textbf{0.1} & \small \textbf{8.8} & \small 0.61 & \small \textbf{0.66} & \small 0.58 \\

\bottomrule
\end{tabular}
\caption{Cross-lingual sentence mining (FLORES-80) and English-only MTEB classification performance.}
\label{tab:merged-eval}
\vspace{-10pt}
\end{table}

\begin{figure}
  \centering
  %left bottom right top
\includegraphics[trim={0cm 0cm 0cm 0cm},clip, width=\columnwidth]{latex/figs/embeddings_layers_full_analysis_mt.pdf}
    \caption{Left: cosine similarity of span pairs across layers. SALT shows a better similarity than SONAR across all layers. Right: translation performance for span embeddings. Both experiments use CrossSpan.}
    \label{span_embeddings}
    \vspace{-10pt}
\end{figure}



\subsection{Analysis}
\label{analysis_sec}

\paragraph{Span embeddings} 
SALT supports span-level representations by averaging token embeddings within each span. We find that these span representations are more semantically informative than their SONAR counterparts. On the CrossSpan test set of high-quality aligned cross-lingual spans, SALT representations of aligned spans consistently exhibit higher cosine similarity across layers (Figure~\ref{span_embeddings}, left), indicating stronger cross-lingual alignment.

A by-product of our span-translation objective is that the learned representations can be directly translated with a \textbf{frozen} SONAR decoder (Figure~\ref{span_embeddings}, right). SALT span embeddings yield high-quality translations, indicating that they preserve rich semantic information for downstream generation. 

\paragraph{Intermediate representations} 
Sentence encoders typically exhibit a \textit{parabolic} behaviour, where intermediate layers achieve the strongest cross-lingual alignment~\citep{simalign}. This arises because cross-lingual token representations emerge in mid-layers but are not necessarily preserved in the final layers, which are more specialised for the pretraining objective. The SALT loss shifts this pattern, with deeper layers becoming more cross-lingually aligned for both spans (Figure~\ref{span_embeddings}, left) and words (Appendix~\ref{word_embeddings_alignment}).

\paragraph{Geometry of the embedding space} We compare the geometry of word embeddings produced by SALT, SONAR, and MEXMA (Table~\ref{geometry_tasks}; see Appendix~\ref{geometry_tasks_exp} for more details on experiments). 

We construct a word retrieval task by merging the datasets from the word alignment task. For each English word, we retrieve the nearest neighbours with cosine similarity and evaluate whether the matches correspond to gold-aligned targets. SALT achieves the highest recall.

A good cross-lingual representation should be language-agnostic, without inducing language-specific subspaces. We probe language separability by training a linear classifier to predict language ID from individual word embeddings. SALT embeddings are significantly harder to classify, indicating more language-invariant representations than SONAR and MEXMA.

Isotropy captures whether the embedding space is dominated by privileged directions, leading to uneven use of representational capacity. We measure it via mean cosine similarity over random word pairs, and via uniformity~\citep{DBLP:conf/icml/0001I20}. MEXMA is highly anisotropic. SONAR and SALT produce more isotropic spaces by these measures, though as we show below, SONAR's apparent isotropy masks a severe hubness problem.

Hubness measures the tendency of a few embeddings to dominate nearest-neighbour retrieval regardless of semantics~\citep{DBLP:journals/jmlr/RadovanovicNI10}. We quantify it via the skewness of the $k$-occurrence distribution, which counts how often an embedding appears in another word's nearest neighbours. Zero skewness indicates a uniform space, while high skewness reflects hub collapse. SONAR exhibits severe hubness (11.5 skewness), while MEXMA and SALT are substantially better behaved. 

Taken together, these results reveal contrasting geometric failures in the baselines. MEXMA produces an anisotropic, language-stratified space, while SONAR suffers from severe hub collapse. SALT avoids both, yielding a better-distributed cross-lingual token space (Figure~\ref{pca}). This suggests that isotropy, hubness and language inseparability are not independent but mutually reinforcing signatures of a well-formed cross-lingual geometry.

\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\begin{tabular}{lcccc}
\toprule
 & \small \textbf{Word Ret. $\uparrow$} & \small \textbf{Lang. ID $\downarrow$} & \small \textbf{Isotropy  $\downarrow$} & \small \textbf{Hub $\downarrow$} \\
\midrule
 &  &  & sim / unif &  \\
MEXMA & 63\% & 0.49 & 0.44 / -2.2 & 4.0 \\
SONAR & 62\% & 0.46 & 0.04 / \textbf{-3.8} & 11.5 \\
SALT  & \textbf{65\%} & \textbf{0.35} & \textbf{0.03} / -3.6 & \textbf{3.5} \\
\bottomrule
\end{tabular}
\caption{Word retrieval (Recall@5), language identification (F1), isotropy (mean cosine similarity and uniformity) and hubness (skewness) for three encoders.}
\label{geometry_tasks}
\vspace{-10pt}
\end{table}


\subsection{Ablations}
\paragraph{Impact of the different losses}
We assess the contribution of each loss term of the SALT training objective by removing them and evaluating across two metrics: word alignment (AER) and averaging the four sequence tagging tasks.

The results are presented in Table~\ref{ablation}. We see that post-training on $\mathcal{L}_{{CON}_{Span}}$ or on $\mathcal{L}_{INT}$ improves on both tasks, being the latest the strongest single loss; $\mathcal{L}_{{MT}_{Span}}$ worsens the pre-trained model, and it worsens word alignment when used in conjunction with $\mathcal{L}_{{CON}_{Span}}$ or on $\mathcal{L}_{INT}$; however, it adds complementary information not fully captured by the other two terms — its inclusion in SALT pushes SeqTag to the best score (0.557), even as $\mathcal{L}_{{CON}_{Span}}+\mathcal{L}_{INT}$ yields a marginally better AER.

The full SALT objective achieves the best sequence tagging score and a highly competitive AER of 0.171, confirming that all three terms are necessary for optimal performance. No subset consistently dominates across both metrics, indicating that each loss captures complementary training signals.

\paragraph{CASE span extraction} Do the SALT improvements stem from an additional external signal, given that LLaMA-70B was used for span extraction? To investigate this, we compare results when training SALT with the self-supervised span extraction heuristic CASE. Results are shown in Table~\ref{llmvslocal}. CASE yields better performance on Massive, whereas external supervision from LLaMA-70B is superior on PAN-X, UDPOS, and WiC. Nevertheless, the difference is marginal: CASE would outperform all the baseline losses and encoders in Table~\ref{main-results} except for UDPOS. This suggests that the training regime is primarily responsible for SALT's success, rather than the span extraction signal itself, and that comparable results can be achieved without access to a strong LLM.

\begin{table}[]
\small
\setlength{\tabcolsep}{3pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
                & \textbf{AER} & \textbf{PAN-X}          & \textbf{Massive}        & \textbf{UDPOS}          & \textbf{WiC}\\
\midrule
SALT (LLaMA) & 0.171          & \textbf{0.622}            & 0.452                       & \textbf{0.571}            & \textbf{0.585}          \\
SALT (CASE)      & 0.171 & 0.613                     & \textbf{0.459}              & 0.568                     & 0.584                 \\
\bottomrule
\end{tabular}}
\caption{Cross-lingual token-level evaluation for SALT using LLaMA-70B spans or the self-supervised CASE.}
\label{llmvslocal}
\end{table}



\begin{table}[]
\setlength{\tabcolsep}{1pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{lcc}
\toprule
                                                                                                 & \small \textbf{AER $\downarrow$}& \small \textbf{SeqTag $\uparrow$}
                                                                                                \\
\midrule
\small SONAR (pre-trained)                                                                                          & \small 0.183        & \small 0.527                   \\
\small $\mathcal{L}_{CON_{Span}}$                                                 &   \small 0.178    &    \small 0.538              \\
\small $\mathcal{L}_{MT_{Span}}$                                                        &   \small   0.186                            & \small    0.522                                     \\
\small $\mathcal{L}_{INT}$                                                              & \small  0.174                               &  \small 0.551                                        \\
\small $\mathcal{L}_{CON_{Span}}    + \mathcal{L}_{MT_{Span}}$ &   \small   0.179                            &   \small  0.551                                     \\
\small $\mathcal{L}_{MT_{Span}} + \mathcal{L}_{INT}$ 

&   \small  0.177                             &   \small  \underline{0.554}                                     \\
\small $\mathcal{L}_{CON_{Span}} + \mathcal{L}_{INT}$         &  \small  \textbf{0.170}                              &  \small      0.552                                  \\
\small
$\mathcal{L}_{CON_{Span}}    + \mathcal{L}_{MT_{Span}} +  \mathcal{L}_{INT}$  (SALT)                                                                                      &   \small  \underline{0.171}                             &       \small \textbf{0.557}           \\                       \bottomrule
\end{tabular}}
\caption{Finetuning SONAR with different losses.}
\label{ablation}
\vspace{-10pt}
\end{table}



==> SALT/latex/6_conclusions.tex <==
\section{Conclusions}
In this work, we introduced SALT, a lightweight post-training method that improves cross-lingual token representations in multilingual sentence encoders through span-aligned supervision. Across multilingual token-level benchmarks, SALT achieved the strongest overall performance, consistently outperforming alternative fine-tuning strategies and competitive encoders. These gains did not come at the expense of sentence-level quality: SALT preserved and, in several cases, improved performance on sentence mining and classification benchmarks. Overall, our results suggest that span-level supervision is a simple yet powerful inductive bias for multilingual representation learning. 

==> SALT/latex/99_ethics.tex <==
\section*{Limitations}
Despite the strong empirical performance of SALT, several limitations remain.

SALT relies on parallel corpora to extract aligned spans, which may limit its applicability to truly low-resource languages. In addition, the self-supervised CASE heuristic assumes that the underlying encoder already provides reasonably good cross-lingual token representations, making adaptation to unseen or severely underrepresented languages more challenging; in those cases, LLM-based spans should be used instead.

Our method also uses average pooling to construct span embeddings. While lightweight and architecture-agnostic, this may fail to capture finer internal structure within longer or compositionally complex spans.

Finally, we only evaluate SALT as a post-training intervention. Exploring span-level supervision during large-scale pre-training could potentially yield larger improvements, but was beyond the computational scope of this work.

\section*{Ethics statement}
This work aims to improve multilingual language representations for token-level cross-lingual tasks, which may help broaden language accessibility and support underrepresented languages in NLP. However, multilingual representation models may also be used in sensitive applications such as surveillance or profiling, and we therefore encourage responsible deployment and evaluation.

Our training data are derived from publicly available parallel corpora from the NLLB Primary dataset, which may contain societal or cultural biases present in web-scale multilingual text. As a result, SALT may inherit biases from the training data or pretrained models.

We also conducted a human evaluation of span quality using native speakers. Participation was voluntary, annotators were informed about the study and their right to withdraw, and no personally identifiable information was collected beyond anonymised annotator IDs. The study received ethics approval from our institution.

==> SALT/latex/miscell.tex <==
\section{Extracting spans with an LLM}
\label{span:extraction}
this is how we do it.


\section{PP}


ace_Arab,ace_Latn,acm_Arab,acq_Arab,aeb_Arab,afr_Latn,ajp_Arab,aka_Latn,amh_Ethi,apc_Arab,arb_Arab,ars_Arab,ary_Arab,arz_Arab,asm_Beng,ast_Latn,awa_Deva,ayr_Latn,azb_Arab,azj_Latn,bak_Cyrl,bam_Latn,ban_Latn,bel_Cyrl,bem_Latn,ben_Beng,bho_Deva,bjn_Arab,bjn_Latn,bod_Tibt,bos_Latn,bug_Latn,bul_Cyrl,cat_Latn,ceb_Latn,ces_Latn,cjk_Latn,ckb_Arab,crh_Latn,cym_Latn,dan_Latn,deu_Latn,dik_Latn,dyu_Latn,dzo_Tibt,ell_Grek,eng_Latn,epo_Latn,est_Latn,eus_Latn,ewe_Latn,fao_Latn,pes_Arab,fij_Latn,fin_Latn,fon_Latn,fra_Latn,fur_Latn,fuv_Latn,gla_Latn,gle_Latn,glg_Latn,grn_Latn,guj_Gujr,hat_Latn,hau_Latn,heb_Hebr,hin_Deva,hne_Deva,hrv_Latn,hun_Latn,hye_Armn,ibo_Latn,ilo_Latn,ind_Latn,isl_Latn,ita_Latn,jav_Latn,jpn_Jpan,kab_Latn,kac_Latn,kam_Latn,kan_Knda,kas_Arab,kas_Deva,kat_Geor,knc_Arab,knc_Latn,kaz_Cyrl,kbp_Latn,kea_Latn,khm_Khmr,kik_Latn,kin_Latn,kir_Cyrl,kmb_Latn,kon_Latn,kor_Hang,kmr_Latn,lao_Laoo,lvs_Latn,lij_Latn,lim_Latn,lin_Latn,lit_Latn,lmo_Latn,ltg_Latn,ltz_Latn,lua_Latn,lug_Latn,luo_Latn,lus_Latn,mag_Deva,mai_Deva,mal_Mlym,mar_Deva,min_Latn,mkd_Cyrl,plt_Latn,mlt_Latn,mni_Beng,khk_Cyrl,mos_Latn,mri_Latn,zsm_Latn,mya_Mymr,nld_Latn,nno_Latn,nob_Latn,npi_Deva,nso_Latn,nus_Latn,nya_Latn,oci_Latn,gaz_Latn,ory_Orya,pag_Latn,pan_Guru,pap_Latn,pol_Latn,por_Latn,prs_Arab,pbt_Arab,quy_Latn,ron_Latn,run_Latn,rus_Cyrl,sag_Latn,san_Deva,sat_Olck,scn_Latn,shn_Mymr,sin_Sinh,slk_Latn,slv_Latn,smo_Latn,sna_Latn,snd_Arab,som_Latn,sot_Latn,spa_Latn,als_Latn,srd_Latn,srp_Cyrl,ssw_Latn,sun_Latn,swe_Latn,swh_Latn,szl_Latn,tam_Taml,tat_Cyrl,tel_Telu,tgk_Cyrl,tgl_Latn,tha_Thai,tir_Ethi,taq_Latn,taq_Tfng,tpi_Latn,tsn_Latn,tso_Latn,tuk_Latn,tum_Latn,tur_Latn,twi_Latn,tzm_Tfng,uig_Arab,ukr_Cyrl,umb_Latn,urd_Arab,uzn_Latn,vec_Latn,vie_Latn,war_Latn,wol_Latn,xho_Latn,ydd_Hebr,yor_Latn,yue_Hant,zho_Hans,zho_Hant,zul_Latn,kur_na,orm_na,pus_na,fas_na,ara_na,tir_ET,msa_na,din_na,aze_na,uzb_na,srp_Latn,bos_Cyrl

['afr_Latn', 'als_Latn', 'amh_Ethi', 'arb_Arab', 'azj_Latn',
       'ben_Beng', 'bul_Cyrl', 'cat_Latn', 'cym_Latn', 'dan_Latn',
       'deu_Latn', 'ell_Grek', 'eng_Latn', 'est_Latn', 'eus_Latn',
       'fin_Latn', 'fra_Latn', 'heb_Hebr', 'hin_Deva', 'hun_Latn',
       'hye_Armn', 'ind_Latn', 'isl_Latn', 'ita_Latn', 'jav_Latn',
       'jpn_Jpan', 'kan_Knda', 'kat_Geor', 'kaz_Cyrl', 'khk_Cyrl',
       'khm_Khmr', 'kor_Hang', 'lvs_Latn', 'mal_Mlym', 'mar_Deva',
       'mya_Mymr', 'nld_Latn', 'nob_Latn', 'pes_Arab', 'pol_Latn',
       'por_Latn', 'ron_Latn', 'rus_Cyrl', 'slv_Latn', 'spa_Latn',
       'swe_Latn', 'swh_Latn', 'tam_Taml', 'tel_Telu', 'tgl_Latn',
       'tha_Thai', 'tur_Latn', 'urd_Arab', 'vie_Latn', 'yor_Latn',
       'zho_Hans', 'zsm_Latn']

source_lang,target_lang,num_rows,blaser2_mean,blaser2_std
por_Latn,zho_Hans,3071,3.0511196854835765,0.41232564851122033
por_Latn,spa_Latn,3071,4.514934737105511,0.36000026339167157
por_Latn,rus_Cyrl,3071,3.8108369090665013,0.4369420477900198
lug_Latn,eng_Latn,15022,4.149441595624122,0.371704447662334
min_Latn,ind_Latn,11571,4.550512195179512,0.3415604840885425
nob_Latn,nno_Latn,40000,4.235276210054756,0.3901313849014885
bam_Latn,eng_Latn,6193,3.686812752882768,0.4049076696743541
aka_Latn,eng_Latn,25420,4.041534537353636,0.4250980239509043
bho_Deva,eng_Latn,6193,4.442375452399504,0.34255110217808715
dzo_Tibt,eng_Latn,6193,3.6176820311430062,0.40267475639127404
som_Latn,tir_Ethi,2030,3.84049536806022,0.4264612726029573
dik_Latn,eng_Latn,6193,3.6161175949708646,0.4405688523506576
eng_Latn,vec_Latn,6193,3.9711865836731284,0.3129462112699098
eng_Latn,fur_Latn,6193,4.1763284601380635,0.31341155104091806
eng_Latn,scn_Latn,6193,3.99513394794498,0.35846852040620175
eng_Latn,hrv_Latn,40000,4.208488458096981,0.4140987504471038
eng_Latn,kas_Deva,6195,3.640772648873687,0.5493151032873287
eng_Latn,fuv_Latn,5171,3.3390615801588983,0.3599604226259132
eng_Latn,pes_Arab,2628,4.4470625370060475,0.22232359152800474
eng_Latn,slv_Latn,40000,4.278917188292742,0.44531756132916017
eng_Latn,urd_Arab,2597,4.28520284949425,0.2600867141823348
eng_Latn,rus_Cyrl,2588,4.529249337762364,0.25342868912522826
eng_Latn,fra_Latn,2721,4.610053613666926,0.27467067559149094
eng_Latn,ukr_Cyrl,40000,4.132498873537779,0.49500841267745616
eng_Latn,tel_Telu,40000,4.035925451037287,0.647083013127817
eng_Latn,hne_Deva,5333,4.340453539291645,0.22066481054804693
eng_Latn,kan_Knda,1860,3.889434734339355,0.3769726969614523
eng_Latn,mag_Deva,5308,4.414639853856217,0.20616557439385919
eng_Latn,tsn_Latn,239,4.57570649789467,0.23611102409083107
eng_Latn,tir_Ethi,749,4.190268462426831,0.314694404158972
eng_Latn,hat_Latn,1356,3.926230397899594,0.28324706714055564
eng_Latn,taq_Latn,5206,3.533239373188041,0.35825340562348634
eng_Latn,ben_Beng,40000,3.8455637452751397,0.6139104081244475
eng_Latn,mni_Beng,5373,4.001360142672503,0.3493354932426507
eng_Latn,knc_Latn,5216,3.4021316256625522,0.3647182907796615
eng_Latn,pbt_Arab,5248,4.151456490658769,0.2714346237891604
eng_Latn,tso_Latn,242,4.483843426073879,0.30439898834162366
eng_Latn,lij_Latn,5278,4.093654146335395,0.22069513644069086
eng_Latn,mri_Latn,5238,3.8638213657158484,0.30304991561726036
eng_Latn,kas_Arab,5229,4.447011971523849,0.24092491698228044
eng_Latn,srd_Latn,5239,4.075002568485765,0.2336220258018023
eng_Latn,grn_Latn,5219,3.740774580883692,0.25116070481479014
eng_Latn,tam_Taml,40000,3.1699862434148787,0.6782416230846067
eng_Latn,prs_Arab,5225,4.280862525091217,0.24037226526314842
eng_Latn,spa_Latn,2676,4.68221274049471,0.22536616346758057
eng_Latn,zho_Hans,2565,4.260645838880632,0.2527280171727732
eng_Latn,knc_Arab,5211,1.9423852835477509,0.3884656387417878
eng_Latn,bos_Latn,40000,4.2362936465084555,0.4065557815608906
eng_Latn,zsm_Latn,2622,4.455379725957444,0.192598330187654
eng_Latn,hin_Deva,40000,4.311031897419691,0.4985918684549044
eng_Latn,bul_Cyrl,40000,4.202303585892916,0.4938415993996823
eng_Latn,ssw_Latn,240,4.206366497278213,0.24708260079091043
eng_Latn,srp_Cyrl,40000,4.112254520434141,0.4082217336703818
eng_Latn,aka_Latn,21283,3.9922590678288112,0.3013496033812211
eng_Latn,por_Latn,2605,4.700218830731002,0.217794766982389
eng_Latn,lug_Latn,12604,4.257103760009416,0.2865521571959109
eng_Latn,som_Latn,1776,4.623486161768973,0.24036215271274727
eng_Latn,mkd_Cyrl,40000,4.219273504731059,0.41675993962695584
eng_Latn,mal_Mlym,40000,3.9941693388313055,0.6264416165819822
eng_Latn,lmo_Latn,5208,4.1142428164841025,0.25281807066178535
eng_Latn,mya_Mymr,2558,4.124674912912012,0.2735355775311205
eng_Latn,sot_Latn,232,4.213451226209772,0.25463898099938514
eng_Latn,ltg_Latn,5239,4.214202642759354,0.23719957577142667
eng_Latn,swh_Latn,2607,4.577019231640429,0.23411702699349649
eng_Latn,shn_Mymr,5184,3.6612616355680387,0.3188788584247453
eng_Latn,ind_Latn,2622,4.488867703146101,0.19716035649199326
eng_Latn,zul_Latn,243,4.309611100718809,0.30837707890716454
eng_Latn,ory_Orya,40000,4.0986373713910575,0.5522230543252667
eng_Latn,yor_Latn,8234,3.8329892578940385,0.48105312203158757
eng_Latn,gaz_Latn,2850,4.024017752680862,0.3094632751129702
eng_Latn,lim_Latn,5217,4.127658776357665,0.2537668062029019
eng_Latn,xho_Latn,239,4.296091884748706,0.27743650894933913
eng_Latn,khm_Khmr,2606,4.047140124662052,0.2419914501507427
eng_Latn,tzm_Tfng,5198,3.3872498150007595,0.34065934006644677
eng_Latn,guj_Gujr,13491,4.078433845547023,0.3226099484721597
eng_Latn,kin_Latn,19341,4.3486809193129545,0.542000437542545
eng_Latn,pan_Guru,626,4.035921653238729,0.31244683073847307
eng_Latn,szl_Latn,5266,4.314115803231769,0.21124604859011947
eng_Latn,nus_Latn,5193,3.4019855435542374,0.3477656942195454
eng_Latn,tgl_Latn,2635,4.428978126098807,0.22003928599132627
eng_Latn,taq_Tfng,5188,3.0983096069341083,0.3995468760566294
yor_Latn,eng_Latn,8274,3.8258287869763024,0.4212846028614245
zul_Latn,eng_Latn,4274,4.141586083143071,0.2846688908392964
ind_Latn,zho_Hans,2573,3.1487283666820503,0.31388290397976376
ind_Latn,spa_Latn,2644,4.475831955175357,0.23290908228757928
ind_Latn,rus_Cyrl,2546,3.817282111740262,0.3285703948835086
ind_Latn,por_Latn,2536,3.7142757236581496,0.34373569223785705
bjn_Latn,eng_Latn,5299,4.517737344337603,0.20734097152980802
crh_Latn,eng_Latn,5193,4.345076651557571,0.25274191347659547
ary_Arab,eng_Latn,5282,4.399933149037331,0.24537946240163322
bjn_Arab,eng_Latn,5227,3.8448762402882055,0.27914413175167024
kin_Latn,eng_Latn,19341,4.452868046092923,0.4898100471996409
nno_Latn,nob_Latn,40000,4.412341017317772,0.386231883409046
gaz_Latn,som_Latn,1720,4.217970916698145,0.2763453570681252
gaz_Latn,tir_Ethi,1719,4.04216585788982,0.3243671318344033
rus_Cyrl,zho_Hans,2563,3.347072186155613,0.30663596078248695
rus_Cyrl,spa_Latn,2606,4.310156452500262,0.2806914345786436
fra_Latn,zul_Latn,2731,4.086706036222326,0.2957192211487781
fra_Latn,ind_Latn,2615,3.5523419154077827,0.3933087118889795
fra_Latn,swh_Latn,2728,4.167038685153306,0.3036139465502004
fra_Latn,por_Latn,2669,4.0287594867583385,0.35014284001968204
fra_Latn,hin_Deva,2616,3.5437999407814913,0.3906041911973774
fra_Latn,spa_Latn,2728,4.357900321134025,0.3226151282577372
fra_Latn,zho_Hans,2616,3.2709451789885122,0.37333178897399805
fra_Latn,ewe_Latn,23663,2.7876884344438926,0.5499147439921873
fra_Latn,lin_Latn,1574,3.238877173451638,0.3774429085021506
fra_Latn,fon_Latn,40000,2.9529481305122376,0.48422018159817154
fra_Latn,rus_Cyrl,2663,3.719507880019282,0.3598616906446826
ace_Latn,eng_Latn,5269,4.3808367241490025,0.2530023854638393
amh_Ethi,eng_Latn,1735,4.202571552837273,0.3189469078013972
amh_Ethi,som_Latn,1712,4.218188538729588,0.28908122157230054
amh_Ethi,gaz_Latn,1698,4.136584756371551,0.3119365030156761
amh_Ethi,tir_Ethi,1714,4.148806876869157,0.33172326205795827
ben_Beng,hin_Deva,2566,4.497636223805666,0.26578026477663513
ben_Beng,eng_Latn,2587,4.086207629079564,0.2442063847680589
fon_Latn,fra_Latn,40000,3.2314836663514375,0.4186275301206689
hat_Latn,eng_Latn,1354,4.023185457753642,0.28342059623779914
ban_Latn,eng_Latn,5288,4.394536010932273,0.2288941449372872
ace_Arab,eng_Latn,5176,3.6934668669560593,0.30995664130961614
arb_Arab,ind_Latn,2528,3.6230020057174226,0.3262474589589081
arb_Arab,eng_Latn,2591,3.9863979438242882,0.2864455857373525
arb_Arab,por_Latn,2594,4.113949426248061,0.2883930422861993
arb_Arab,hin_Deva,2536,3.848082337375695,0.3773549718951038
arb_Arab,zho_Hans,2562,3.3977483020547217,0.3185117047650182
arb_Arab,spa_Latn,2588,4.145627215343429,0.27677434827683517
arb_Arab,fra_Latn,2680,4.031564870254317,0.31432570462520115
arb_Arab,rus_Cyrl,2572,4.1804497009302555,0.3177903405529044
arz_Arab,eng_Latn,5265,4.423121398262828,0.22508792985935164
ewe_Latn,fra_Latn,23663,3.0320375377960684,0.4932316269394934
afr_Latn,eng_Latn,249,4.527302517948381,0.23637567473052423
lin_Latn,fra_Latn,1568,3.2575835249557787,0.37463095035280847
hin_Deva,por_Latn,2549,3.8136906840839586,0.3323440404622098
hin_Deva,ind_Latn,2516,3.8829680933292794,0.3104118688091974
hin_Deva,mar_Deva,2559,4.506248434431249,0.2852819872209007
hin_Deva,rus_Cyrl,2562,3.9322676090036492,0.3016440258397486
hin_Deva,urd_Arab,2579,4.345092108657352,0.28815732178343784
hin_Deva,zho_Hans,2587,3.408871390619562,0.3298230613877395
hin_Deva,spa_Latn,2597,4.385341685783143,0.25680995083959396
bug_Latn,eng_Latn,5255,4.254177651963384,0.26373128166709203
spa_Latn,zho_Hans,2559,3.378832588721272,0.33456526923003893

==> latex/1_intro_old.tex <==
%%%%%%% IGNORE!!


\section{Introduction}
While modern cross-lingual encoders excel at aligning sentences across languages, their behaviour at finer levels of linguistic structure remains largely unexplored. In particular, little is known about whether cross-lingual alignment consistently emerges at the level of phrases and individual tokens.

%Two sentences may share similar representations, even if the words and phrases that compose them are poorly aligned across languages.




-> fer un exemple on hi hagi un poor alignment!!!!! 






. Early research focused on the development of static word embeddings or token representations~\citep{DBLP:conf/nips/BengioDV00, word2vec, glove, fasttext}. 


The advent of Masked Language Modeling (MLM) enabled models to generate contextual word embeddings that capture nuanced meaning based on surrounding text~\citep{bert}. This foundation was extended to the multilingual setting, resulting in models such as M-BERT and XLM that are trained on corpora from multiple languages~\citep{bert, xlm} to facilitate knowledge transfer across languages. This improved performance on cross-lingual tasks, although certain challenges—such as effective alignment of words and handling of low-resource languages remain.

Recent efforts in building strong cross-lingual representations have focus at the \textit{sentence} level~\citep{laser, labse, sonar, mexma, sonar2}. This has advantages for [...]. 

[TOKEN EMBEDDINGS ARE PRACTICALLY IMPORTANT: MTQE, SEQ TAGGING, LABEL EXTRAP.]

However, we a current limitation. 

[WHAT WE DO HERE]

We focus on the three key research questions (RQs): (i) Do sentence embedders preserve local information that is usable for token-rich tasks? (ii) Can additional unsupervised training objective enhance these properties while preserving the sentence-level space? (iii) What are the trade-offs between an improved local (token-level) and global (sentence-level) alignments? 

The key contributions of this work are:
\begin{itemize}
    \item We study token embeddings of sentence representations. 
    \item We study using losses to improve the local representations. We study the trade-offs. 
\end{itemize}

==> latex/1_intro_oldold.tex <==

%%%%%%% IGNORE!!



\newpage
Multilingual sentence encoders have become a central component of cross-lingual NLP. Models such as SONAR~\citep{sonar} or MEXMA~\citep{mexma} learn a shared embedding space in which semantically equivalent sentences across languages are mapped to nearby representations, achieving strong performance on tasks such as cross-lingual retrieval, sentence mining, and zero-shot classification.

While sentence-level alignment is explicitly optimised during training, these models are often repurposed as token encoders despite never being trained for this setting. This creates a structural mismatch: sentence encoders are supervised to preserve global semantic similarity, yet are widely used in tasks that depend on fine-grained token- and span-level correspondence. As a result, they may produce well-structured sentence embeddings while still exhibiting weak or inconsistent token-level alignment. In practice, many downstream applications rely on token embeddings derived from sentence encoders, including word alignment~\citep{simalign}, sequence tagging~\citep{peters-etal-2017-semi}, hallucination detection~\citep{ottawa} or label projection~\citep{labelproj}.

In this work, we investigate whether the token representations of multilingual sentence encoders can be improved through additional training objectives that operate at a finer granularity. We argue that sentence-level translation data implicitly encodes \textit{span}-level alignment structure that is systematically ignored by standard training objectives.

Our key observation is that translation pairs provide a natural signal not only at the sentence level but also at the lower level of \emph{spans}—contiguous sequences of tokens that express equivalent meaning across languages (see Figure~\ref{diagram}). This signal allows us to directly encourage the alignment of semantically corresponding phrases while maintaining the global structure of the sentence embedding space.

To this end, we propose \salt{0.05} \textbf{SALT} (\textbf{S}pan-\textbf{A}ligned \textbf{L}earning for cross-lingual \textbf{T}okens), a lightweight post-training procedure for multilingual sentence encoders. SALT introduces span-level contrastive and translation objectives to refine token representations, alongside a sentence-level interpolation loss that preserves the original embedding space. Crucially, SALT can be applied to an existing sentence encoder without architectural modifications and is compatible with decoders produced during pre-training.

We evaluate SALT on a suite of multilingual token-level benchmarks, including word alignment, cross-lingual sequence tagging and word sense disambiguation. SALT consistently improves token-level performance while maintaining strong sentence-level representations. In particular, SALT achieves the best overall performance among several alternative fine-tuning strategies on four out of five token-level benchmarks. At the same time, sentence-level evaluation shows that the method preserves--and in some cases improves--the quality of the original embedding space.

Our contributions are the following:

\begin{itemize}
%\item We introduce SALT, a span-aligned post-training method that improves cross-lingual token representations while preserving sentence-level alignment. SALT can use either local or external alignments. 
%\item We demonstrate that our span-level supervision provides a complementary training signal that leads to consistent improvements across multiple multilingual tasks.

\item We propose \textbf{SALT}, a lightweight post-training method that improves cross-lingual token representations via span-aligned objectives.

\item SALT consistently improves performance in multiple token-level multilingual tasks, including word alignment, sequence tagging, and word sense disambiguation, while improving sentence-level performance.

\item SALT is flexible and plug-and-play, supporting both automatically induced (local) and externally provided span alignments, and can be applied to existing sentence encoders and decoders without architectural modifications.
\end{itemize}


==> latex/4_experiments_old.tex <==
Table~\ref{alignment}
Table~\ref{best_layer}

\begin{table*}[]
\centering
{\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
                   & \textbf{Average}   & \textbf{de-en} & \textbf{en-bg} & \textbf{en-cs} & \textbf{en-da} & \textbf{en-es} & \textbf{en-et} & \textbf{en-fa} & \textbf{en-fr} & \textbf{en-hi} & \textbf{en-hu} & \textbf{en-it} & \textbf{en-nl} & \textbf{en-pt} & \textbf{en-ru} & \textbf{en-sl} & \textbf{ja-en} & \textbf{ro-en} & \textbf{zh-en} \\
                   \midrule
\footnotesize XLM-Roberta & 0.203          & 0.192          & 0.147          & 0.126          & 0.093          & 0.144          & 0.195          & 0.308          & 0.064          & 0.379          & 0.214          & 0.189          & 0.072          & 0.149          & 0.147          & 0.185          & 0.503          & 0.258          & 0.288          \\
\footnotesize XLM-v       & 0.206          & 0.188          & 0.146          & 0.123          & 0.102          & 0.137          & 0.184          & 0.311          & 0.063          & 0.383          & 0.208          & 0.185          & 0.067          & 0.143          & 0.156          & 0.18           & 0.532          & 0.268          & 0.326          \\
\footnotesize XLM-Align   & 0.184          & 0.167          & 0.13           & 0.106          & 0.085          & 0.129          & 0.185          & 0.289          & 0.056          & 0.328          & 0.205          & 0.17           & 0.062          & 0.135          & 0.134          & 0.176          & 0.455          & 0.253          & 0.242          \\
\footnotesize MEXMA              & \textbf{0.166} & \textbf{0.163} & \textbf{0.124} & \textbf{0.091} & \textbf{0.074} & \textbf{0.119} & \textbf{0.148} & \textbf{0.251} & \textbf{0.047} & \textbf{0.292} & \textbf{0.193} & \textbf{0.163} & \textbf{0.05}  & \textbf{0.131} & \textbf{0.126} & 0.161          & \textbf{0.428} & 0.217          & 0.212          \\
\footnotesize SONARv1            & 0.174          & 0.184          & 0.131          & 0.095          & 0.081          & 0.123          & 0.159          & 0.268          & 0.054          & 0.3            & 0.206          & 0.174          & 0.065          & 0.136          & 0.129          & \textbf{0.158} & 0.441          & \textbf{0.216} & \textbf{0.207} \\
\footnotesize SONARv2            & 0.19           & 0.207          & 0.14           & 0.119          & 0.089          & 0.144          & 0.166          & 0.297          & 0.071          & 0.326          & 0.216          & 0.19           & 0.074          & 0.143          & 0.148          & 0.185          & 0.443          & 0.251          & 0.22           \\
\footnotesize SONAR-Omni         & 0.192          & 0.207          & 0.138          & 0.114          & 0.094          & 0.144          & 0.167          & 0.307          & 0.071          & 0.315          & 0.221          & 0.187          & 0.072          & 0.14           & 0.152          & 0.185          & 0.449          & 0.256          & 0.23          
\\
\bottomrule
\end{tabular}}
\caption{AER for }
\label{alignment}
\end{table*}


\begin{table}[]
\centering
{
\begin{tabular}{lcc}
\toprule
                   & \multicolumn{1}{l}{Best} & \multicolumn{1}{l}{Average} \\
                   \midrule
XLM-Roberta & 8                              & 0.203                \\
XLM-v      & 7                              & 0.201                   \\
XLM-Align & 8                              & 0.184                   \\
MEXMA              & 20                             & 0.163                   \\
SONARv1            & 19                             & 0.161                   \\
SONARv2            & 8                              & 0.165                   \\
SONAR-Omni         & 8                              & 0.167                  \\
\bottomrule
\end{tabular} }
\caption{AER for }
\label{best_layer}
\end{table}





\subsection{Sequence tagging}
Table~\ref{seq:label}
\begin{table*}[]
\centering
{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccccc}
\toprule
& \shortstack{Massive \\ {\small (English)}}
& \shortstack{Massive \\ {\small (All)}}
& \shortstack{Massive \\ {\small (Single)}}
& \shortstack{PAN-X \\ {\small (English)}}
& \shortstack{PAN-X \\ {\small (All)}} & \shortstack{PAN-X \\ {\small (Single)}}
& \shortstack{UDPOS \\ {\small (English)}}
& \shortstack{UDPOS \\ {\small (All)}} & \shortstack{UDPOS \\ {\small (Single)}}\\
\midrule
mBERT       & 0.142                                                                                          & 0.306                                                                                      & 0.458                & 0.576                                                                                        & 0.695                                                                                    & 0.812                & 0.426                                                                                        & 0.565                                                                                    & 0.718                \\
XLM-Roberta & 0.230                                                                                          & 0.410                                                                                      & 0.468                & 0.546                                                                                        & 0.640                                                                                    & 0.762                & 0.507                                                                                        & 0.617                                                                                    & 0.763                \\
XLM-v       & 0.269                                                                                          & 0.480                                                                                      & 0.495                & 0.594                                                                                        & 0.692                                                                                    & 0.786                & \textbf{0.528}                                                                               & \textbf{0.634}                                                                           & 0.755                \\
MEXMA       & 0.454                                                                                          & 0.599                                                                                      & \textbf{0.573}       & 0.611                                                                                        & 0.708                                                                                    & \textbf{0.819}                & 0.522                                                                                        & 0.593                                                                                    & \textbf{0.764}       \\
SONARv1     & 0.446                                                                                          & 0.574                                                                                      & 0.561                & 0.594                                                                                        & 0.698                                                                                    & 0.805                & 0.522                                                                                        & 0.565                                                                                    & 0.720                \\
SONARv2     & \textbf{0.490}                                                                                 & 0.602                                                                                      & 0.567                & 0.616                                                                                        & \textbf{0.716}                                                                           & 0.817       & 0.519                                                                                        & 0.585                                                                                    & 0.750                \\
SONAR-Omni  & 0.479                                                                                          & \textbf{0.607}                                                                             & 0.567                & \textbf{0.624}                                                                               & 0.710                                                                                    & 0.809                & 0.520                                                                                        & 0.580                                                                                    & 0.725                \\ 
\bottomrule                   
\end{tabular} }
\caption{blabla}
\label{seq:label}
\end{table*}





\begin{table*}[]
\centering
{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
& \shortstack{Massive \\ {\small (English)}}
& \shortstack{Massive \\ {\small (All)}}
& \shortstack{PAN-X \\ {\small (English)}}
& \shortstack{PAN-X \\ {\small (All)}}
& \shortstack{UDPOS \\ {\small (English)}}
& \shortstack{UDPOS \\ {\small (All)}} \\
\midrule
MEXMA            & 0.454                                                                                          & 0.599                                                                                      & 0.611                                                                                        & 0.708                                                                                    & 0.522                                                                                        & 0.593                                                                                    \\
SONARv1 (frozen) & 0.446                                                                                          & 0.574                                                                                      & 0.594                                                                                        & 0.698                                                                                    & 0.522                                                                                        & 0.565                                                                                    \\
Teacher Loss     & 0.478                                                                                          & 0.589                                                                                      & 0.606                                                                                        & 0.711                                                                                    & 0.502                                                                                        & 0.561                                                                                    \\
SO (R=0.3)       & 0.461                                                                                          & 0.586                                                                                      & 0.607                                                                                        & 0.709                                                                                    & 0.527                                                                                        & 0.577                                                                                    \\
SONARv2          & \textbf{0.490}                                                                                 & 0.602                                                                                      & 0.616                                                                                        & \textbf{0.716}                                                                           & 0.519                                                                                        & 0.585                                                                                    \\
SONAR-Omni       & 0.479                                                                                          & \textbf{0.607}                                                                             & \textbf{0.624}                                                                               & 0.710                                                                                    & 0.520                                                                                        & 0.580                                                                                    \\
\bottomrule                   
\end{tabular} }
\caption{blabla}
\label{seq:label}
\end{table*}




\subsection{Machine Translation Quality Estimation}

==> latex/miscell.tex <==
\section{Extracting spans with an LLM}
\label{span:extraction}
this is how we do it.


\section{PP}


ace_Arab,ace_Latn,acm_Arab,acq_Arab,aeb_Arab,afr_Latn,ajp_Arab,aka_Latn,amh_Ethi,apc_Arab,arb_Arab,ars_Arab,ary_Arab,arz_Arab,asm_Beng,ast_Latn,awa_Deva,ayr_Latn,azb_Arab,azj_Latn,bak_Cyrl,bam_Latn,ban_Latn,bel_Cyrl,bem_Latn,ben_Beng,bho_Deva,bjn_Arab,bjn_Latn,bod_Tibt,bos_Latn,bug_Latn,bul_Cyrl,cat_Latn,ceb_Latn,ces_Latn,cjk_Latn,ckb_Arab,crh_Latn,cym_Latn,dan_Latn,deu_Latn,dik_Latn,dyu_Latn,dzo_Tibt,ell_Grek,eng_Latn,epo_Latn,est_Latn,eus_Latn,ewe_Latn,fao_Latn,pes_Arab,fij_Latn,fin_Latn,fon_Latn,fra_Latn,fur_Latn,fuv_Latn,gla_Latn,gle_Latn,glg_Latn,grn_Latn,guj_Gujr,hat_Latn,hau_Latn,heb_Hebr,hin_Deva,hne_Deva,hrv_Latn,hun_Latn,hye_Armn,ibo_Latn,ilo_Latn,ind_Latn,isl_Latn,ita_Latn,jav_Latn,jpn_Jpan,kab_Latn,kac_Latn,kam_Latn,kan_Knda,kas_Arab,kas_Deva,kat_Geor,knc_Arab,knc_Latn,kaz_Cyrl,kbp_Latn,kea_Latn,khm_Khmr,kik_Latn,kin_Latn,kir_Cyrl,kmb_Latn,kon_Latn,kor_Hang,kmr_Latn,lao_Laoo,lvs_Latn,lij_Latn,lim_Latn,lin_Latn,lit_Latn,lmo_Latn,ltg_Latn,ltz_Latn,lua_Latn,lug_Latn,luo_Latn,lus_Latn,mag_Deva,mai_Deva,mal_Mlym,mar_Deva,min_Latn,mkd_Cyrl,plt_Latn,mlt_Latn,mni_Beng,khk_Cyrl,mos_Latn,mri_Latn,zsm_Latn,mya_Mymr,nld_Latn,nno_Latn,nob_Latn,npi_Deva,nso_Latn,nus_Latn,nya_Latn,oci_Latn,gaz_Latn,ory_Orya,pag_Latn,pan_Guru,pap_Latn,pol_Latn,por_Latn,prs_Arab,pbt_Arab,quy_Latn,ron_Latn,run_Latn,rus_Cyrl,sag_Latn,san_Deva,sat_Olck,scn_Latn,shn_Mymr,sin_Sinh,slk_Latn,slv_Latn,smo_Latn,sna_Latn,snd_Arab,som_Latn,sot_Latn,spa_Latn,als_Latn,srd_Latn,srp_Cyrl,ssw_Latn,sun_Latn,swe_Latn,swh_Latn,szl_Latn,tam_Taml,tat_Cyrl,tel_Telu,tgk_Cyrl,tgl_Latn,tha_Thai,tir_Ethi,taq_Latn,taq_Tfng,tpi_Latn,tsn_Latn,tso_Latn,tuk_Latn,tum_Latn,tur_Latn,twi_Latn,tzm_Tfng,uig_Arab,ukr_Cyrl,umb_Latn,urd_Arab,uzn_Latn,vec_Latn,vie_Latn,war_Latn,wol_Latn,xho_Latn,ydd_Hebr,yor_Latn,yue_Hant,zho_Hans,zho_Hant,zul_Latn,kur_na,orm_na,pus_na,fas_na,ara_na,tir_ET,msa_na,din_na,aze_na,uzb_na,srp_Latn,bos_Cyrl

['afr_Latn', 'als_Latn', 'amh_Ethi', 'arb_Arab', 'azj_Latn',
       'ben_Beng', 'bul_Cyrl', 'cat_Latn', 'cym_Latn', 'dan_Latn',
       'deu_Latn', 'ell_Grek', 'eng_Latn', 'est_Latn', 'eus_Latn',
       'fin_Latn', 'fra_Latn', 'heb_Hebr', 'hin_Deva', 'hun_Latn',
       'hye_Armn', 'ind_Latn', 'isl_Latn', 'ita_Latn', 'jav_Latn',
       'jpn_Jpan', 'kan_Knda', 'kat_Geor', 'kaz_Cyrl', 'khk_Cyrl',
       'khm_Khmr', 'kor_Hang', 'lvs_Latn', 'mal_Mlym', 'mar_Deva',
       'mya_Mymr', 'nld_Latn', 'nob_Latn', 'pes_Arab', 'pol_Latn',
       'por_Latn', 'ron_Latn', 'rus_Cyrl', 'slv_Latn', 'spa_Latn',
       'swe_Latn', 'swh_Latn', 'tam_Taml', 'tel_Telu', 'tgl_Latn',
       'tha_Thai', 'tur_Latn', 'urd_Arab', 'vie_Latn', 'yor_Latn',
       'zho_Hans', 'zsm_Latn']

source_lang,target_lang,num_rows,blaser2_mean,blaser2_std
por_Latn,zho_Hans,3071,3.0511196854835765,0.41232564851122033
por_Latn,spa_Latn,3071,4.514934737105511,0.36000026339167157
por_Latn,rus_Cyrl,3071,3.8108369090665013,0.4369420477900198
lug_Latn,eng_Latn,15022,4.149441595624122,0.371704447662334
min_Latn,ind_Latn,11571,4.550512195179512,0.3415604840885425
nob_Latn,nno_Latn,40000,4.235276210054756,0.3901313849014885
bam_Latn,eng_Latn,6193,3.686812752882768,0.4049076696743541
aka_Latn,eng_Latn,25420,4.041534537353636,0.4250980239509043
bho_Deva,eng_Latn,6193,4.442375452399504,0.34255110217808715
dzo_Tibt,eng_Latn,6193,3.6176820311430062,0.40267475639127404
som_Latn,tir_Ethi,2030,3.84049536806022,0.4264612726029573
dik_Latn,eng_Latn,6193,3.6161175949708646,0.4405688523506576
eng_Latn,vec_Latn,6193,3.9711865836731284,0.3129462112699098
eng_Latn,fur_Latn,6193,4.1763284601380635,0.31341155104091806
eng_Latn,scn_Latn,6193,3.99513394794498,0.35846852040620175
eng_Latn,hrv_Latn,40000,4.208488458096981,0.4140987504471038
eng_Latn,kas_Deva,6195,3.640772648873687,0.5493151032873287
eng_Latn,fuv_Latn,5171,3.3390615801588983,0.3599604226259132
eng_Latn,pes_Arab,2628,4.4470625370060475,0.22232359152800474
eng_Latn,slv_Latn,40000,4.278917188292742,0.44531756132916017
eng_Latn,urd_Arab,2597,4.28520284949425,0.2600867141823348
eng_Latn,rus_Cyrl,2588,4.529249337762364,0.25342868912522826
eng_Latn,fra_Latn,2721,4.610053613666926,0.27467067559149094
eng_Latn,ukr_Cyrl,40000,4.132498873537779,0.49500841267745616
eng_Latn,tel_Telu,40000,4.035925451037287,0.647083013127817
eng_Latn,hne_Deva,5333,4.340453539291645,0.22066481054804693
eng_Latn,kan_Knda,1860,3.889434734339355,0.3769726969614523
eng_Latn,mag_Deva,5308,4.414639853856217,0.20616557439385919
eng_Latn,tsn_Latn,239,4.57570649789467,0.23611102409083107
eng_Latn,tir_Ethi,749,4.190268462426831,0.314694404158972
eng_Latn,hat_Latn,1356,3.926230397899594,0.28324706714055564
eng_Latn,taq_Latn,5206,3.533239373188041,0.35825340562348634
eng_Latn,ben_Beng,40000,3.8455637452751397,0.6139104081244475
eng_Latn,mni_Beng,5373,4.001360142672503,0.3493354932426507
eng_Latn,knc_Latn,5216,3.4021316256625522,0.3647182907796615
eng_Latn,pbt_Arab,5248,4.151456490658769,0.2714346237891604
eng_Latn,tso_Latn,242,4.483843426073879,0.30439898834162366
eng_Latn,lij_Latn,5278,4.093654146335395,0.22069513644069086
eng_Latn,mri_Latn,5238,3.8638213657158484,0.30304991561726036
eng_Latn,kas_Arab,5229,4.447011971523849,0.24092491698228044
eng_Latn,srd_Latn,5239,4.075002568485765,0.2336220258018023
eng_Latn,grn_Latn,5219,3.740774580883692,0.25116070481479014
eng_Latn,tam_Taml,40000,3.1699862434148787,0.6782416230846067
eng_Latn,prs_Arab,5225,4.280862525091217,0.24037226526314842
eng_Latn,spa_Latn,2676,4.68221274049471,0.22536616346758057
eng_Latn,zho_Hans,2565,4.260645838880632,0.2527280171727732
eng_Latn,knc_Arab,5211,1.9423852835477509,0.3884656387417878
eng_Latn,bos_Latn,40000,4.2362936465084555,0.4065557815608906
eng_Latn,zsm_Latn,2622,4.455379725957444,0.192598330187654
eng_Latn,hin_Deva,40000,4.311031897419691,0.4985918684549044
eng_Latn,bul_Cyrl,40000,4.202303585892916,0.4938415993996823
eng_Latn,ssw_Latn,240,4.206366497278213,0.24708260079091043
eng_Latn,srp_Cyrl,40000,4.112254520434141,0.4082217336703818
eng_Latn,aka_Latn,21283,3.9922590678288112,0.3013496033812211
eng_Latn,por_Latn,2605,4.700218830731002,0.217794766982389
eng_Latn,lug_Latn,12604,4.257103760009416,0.2865521571959109
eng_Latn,som_Latn,1776,4.623486161768973,0.24036215271274727
eng_Latn,mkd_Cyrl,40000,4.219273504731059,0.41675993962695584
eng_Latn,mal_Mlym,40000,3.9941693388313055,0.6264416165819822
eng_Latn,lmo_Latn,5208,4.1142428164841025,0.25281807066178535
eng_Latn,mya_Mymr,2558,4.124674912912012,0.2735355775311205
eng_Latn,sot_Latn,232,4.213451226209772,0.25463898099938514
eng_Latn,ltg_Latn,5239,4.214202642759354,0.23719957577142667
eng_Latn,swh_Latn,2607,4.577019231640429,0.23411702699349649
eng_Latn,shn_Mymr,5184,3.6612616355680387,0.3188788584247453
eng_Latn,ind_Latn,2622,4.488867703146101,0.19716035649199326
eng_Latn,zul_Latn,243,4.309611100718809,0.30837707890716454
eng_Latn,ory_Orya,40000,4.0986373713910575,0.5522230543252667
eng_Latn,yor_Latn,8234,3.8329892578940385,0.48105312203158757
eng_Latn,gaz_Latn,2850,4.024017752680862,0.3094632751129702
eng_Latn,lim_Latn,5217,4.127658776357665,0.2537668062029019
eng_Latn,xho_Latn,239,4.296091884748706,0.27743650894933913
eng_Latn,khm_Khmr,2606,4.047140124662052,0.2419914501507427
eng_Latn,tzm_Tfng,5198,3.3872498150007595,0.34065934006644677
eng_Latn,guj_Gujr,13491,4.078433845547023,0.3226099484721597
eng_Latn,kin_Latn,19341,4.3486809193129545,0.542000437542545
eng_Latn,pan_Guru,626,4.035921653238729,0.31244683073847307
eng_Latn,szl_Latn,5266,4.314115803231769,0.21124604859011947
eng_Latn,nus_Latn,5193,3.4019855435542374,0.3477656942195454
eng_Latn,tgl_Latn,2635,4.428978126098807,0.22003928599132627
eng_Latn,taq_Tfng,5188,3.0983096069341083,0.3995468760566294
yor_Latn,eng_Latn,8274,3.8258287869763024,0.4212846028614245
zul_Latn,eng_Latn,4274,4.141586083143071,0.2846688908392964
ind_Latn,zho_Hans,2573,3.1487283666820503,0.31388290397976376
ind_Latn,spa_Latn,2644,4.475831955175357,0.23290908228757928
ind_Latn,rus_Cyrl,2546,3.817282111740262,0.3285703948835086
ind_Latn,por_Latn,2536,3.7142757236581496,0.34373569223785705
bjn_Latn,eng_Latn,5299,4.517737344337603,0.20734097152980802
crh_Latn,eng_Latn,5193,4.345076651557571,0.25274191347659547
ary_Arab,eng_Latn,5282,4.399933149037331,0.24537946240163322
bjn_Arab,eng_Latn,5227,3.8448762402882055,0.27914413175167024
kin_Latn,eng_Latn,19341,4.452868046092923,0.4898100471996409
nno_Latn,nob_Latn,40000,4.412341017317772,0.386231883409046
gaz_Latn,som_Latn,1720,4.217970916698145,0.2763453570681252
gaz_Latn,tir_Ethi,1719,4.04216585788982,0.3243671318344033
rus_Cyrl,zho_Hans,2563,3.347072186155613,0.30663596078248695
rus_Cyrl,spa_Latn,2606,4.310156452500262,0.2806914345786436
fra_Latn,zul_Latn,2731,4.086706036222326,0.2957192211487781
fra_Latn,ind_Latn,2615,3.5523419154077827,0.3933087118889795
fra_Latn,swh_Latn,2728,4.167038685153306,0.3036139465502004
fra_Latn,por_Latn,2669,4.0287594867583385,0.35014284001968204
fra_Latn,hin_Deva,2616,3.5437999407814913,0.3906041911973774
fra_Latn,spa_Latn,2728,4.357900321134025,0.3226151282577372
fra_Latn,zho_Hans,2616,3.2709451789885122,0.37333178897399805
fra_Latn,ewe_Latn,23663,2.7876884344438926,0.5499147439921873
fra_Latn,lin_Latn,1574,3.238877173451638,0.3774429085021506
fra_Latn,fon_Latn,40000,2.9529481305122376,0.48422018159817154
fra_Latn,rus_Cyrl,2663,3.719507880019282,0.3598616906446826
ace_Latn,eng_Latn,5269,4.3808367241490025,0.2530023854638393
amh_Ethi,eng_Latn,1735,4.202571552837273,0.3189469078013972
amh_Ethi,som_Latn,1712,4.218188538729588,0.28908122157230054
amh_Ethi,gaz_Latn,1698,4.136584756371551,0.3119365030156761
amh_Ethi,tir_Ethi,1714,4.148806876869157,0.33172326205795827
ben_Beng,hin_Deva,2566,4.497636223805666,0.26578026477663513
ben_Beng,eng_Latn,2587,4.086207629079564,0.2442063847680589
fon_Latn,fra_Latn,40000,3.2314836663514375,0.4186275301206689
hat_Latn,eng_Latn,1354,4.023185457753642,0.28342059623779914
ban_Latn,eng_Latn,5288,4.394536010932273,0.2288941449372872
ace_Arab,eng_Latn,5176,3.6934668669560593,0.30995664130961614
arb_Arab,ind_Latn,2528,3.6230020057174226,0.3262474589589081
arb_Arab,eng_Latn,2591,3.9863979438242882,0.2864455857373525
arb_Arab,por_Latn,2594,4.113949426248061,0.2883930422861993
arb_Arab,hin_Deva,2536,3.848082337375695,0.3773549718951038
arb_Arab,zho_Hans,2562,3.3977483020547217,0.3185117047650182
arb_Arab,spa_Latn,2588,4.145627215343429,0.27677434827683517
arb_Arab,fra_Latn,2680,4.031564870254317,0.31432570462520115
arb_Arab,rus_Cyrl,2572,4.1804497009302555,0.3177903405529044
arz_Arab,eng_Latn,5265,4.423121398262828,0.22508792985935164
ewe_Latn,fra_Latn,23663,3.0320375377960684,0.4932316269394934
afr_Latn,eng_Latn,249,4.527302517948381,0.23637567473052423
lin_Latn,fra_Latn,1568,3.2575835249557787,0.37463095035280847
hin_Deva,por_Latn,2549,3.8136906840839586,0.3323440404622098
hin_Deva,ind_Latn,2516,3.8829680933292794,0.3104118688091974
hin_Deva,mar_Deva,2559,4.506248434431249,0.2852819872209007
hin_Deva,rus_Cyrl,2562,3.9322676090036492,0.3016440258397486
hin_Deva,urd_Arab,2579,4.345092108657352,0.28815732178343784
hin_Deva,zho_Hans,2587,3.408871390619562,0.3298230613877395
hin_Deva,spa_Latn,2597,4.385341685783143,0.25680995083959396
bug_Latn,eng_Latn,5255,4.254177651963384,0.26373128166709203
spa_Latn,zho_Hans,2559,3.378832588721272,0.33456526923003893
